An Empirical Study on Logging Evolution On Stack Overflow: Trends, Topics, and Challenges

Context: Logging is a crucial practice in software engineering, aiding developers in debugging applications when errors occur. While existing research has explored logging challenges from an academic perspective through literature reviews and source code analysis, a comprehensive study from the practitioners' perspective remains lacking. Objective: This paper aims to bridge this knowledge gap by presenting an in-depth analysis of trends, topics, and challenges in logging based on a dataset of 216,094 posts from Stack Overflow (SO), a popular Q\&A platform for developers. Method: We analyzed longitudinal trends by examining metadata related to users, questions, and tags associated with logging discussions. To identify prevalent discussion topics, we employed a Large Language Model (LLM)--based classification approach, based on a manually validated ground-truth sample. Topic popularity was assessed through average scores and views, while difficulty was measured using three community-driven metrics: the proportion of questions without accepted answers, the proportion of unanswered questions, and the median time to receive an accepted answer. Results: Our analysis identifies 11 distinct topics, with the top three (General Logging Practices, Error Handling and Debugging, and Logging Levels and Output) accounting for over 70\% of all logging-related discussions. Notably, Logging in Containerized Environments emerged as the most difficult topic: 64.9\% of its questions lack an accepted answer, and its median resolution time is among the highest. These findings highlight enduring practitioner struggles with logging in Docker or other containerized environments and the integration of logging pipelines into orchestrators such as Kubernetes and cloud environments. Conclusion: This study sheds light on the practical challenges of logging and provides actionable insights for developers, framework vendors, researchers, and educators.

==> 0_Preamble.tex <==
% First comes an example EPS file -- just ignore it and
% proceed on the \documentclass line
% your LaTeX will extract the file if required
% \begin{filecontents*}{example.eps}

% %%BoundingBox: 19 19 221 221
% %%CreationDate: Mon Sep 29 1997
% %%Creator: programmed by hand (JK)
% %%EndComments
% gsave
% newpath
%   20 20 moveto
%   20 220 lineto
%   220 220 lineto
%   220 20 lineto
% closepath
% 2 setlinewidth
% gsave
%   .4 setgray fill
% grestore
% stroke
% grestore
% \end{filecontents*}
%
\RequirePackage{fix-cm}

% Need To Remove Before Submit
\AtBeginDocument{%
  \paperwidth=\dimexpr
    1in + \oddsidemargin
    + \textwidth
    % + \marginparsep + \marginparwidth
    + 1in + \oddsidemargin
  \relax
  \paperheight=\dimexpr
    1in + \topmargin
    + \headheight + \headsep
    + \textheight
    % + \footskip
    + 1in + \topmargin
  \relax
  \usepackage[pass]{geometry}\relax
}
% ---------------------------------------------------------------------------------------------------------------------------
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{soul}	
\usepackage{balance}
\usepackage{tabularx}
\usepackage{enumitem}
\usepackage{adjustbox}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{caption}
\usepackage{hyperref}
\usepackage{dirtytalk} 
\usepackage{xcolor}
\usepackage{xcolor}
\usepackage[most]{tcolorbox}
\usepackage{pifont}
\usepackage[mathlines,switch]{lineno}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{%
            \node[shape=circle,draw,inner sep=1pt] (char) {#1};}}
\usepackage{tikz}
% ---------------------------------------------------------------------------------------------------------------------------
%
\usepackage{graphicx}
\usepackage{listings}
% \usepackage{color}
\usepackage{pifont}
\usepackage{amsmath}
\usepackage{pdflscape} 
\usepackage{tikz}
\usepackage{dirtytalk}
\usepackage{makecell}
\usepackage[title]{appendix}
\usepackage{pythonhighlight}
%\usepackage[newfloat]{minted}
\usepackage{caption}
\newenvironment{code}{\captionsetup{type=listing}}{}
%\SetupFloatingEnvironment{listing}{name=Source Code}
% \usepackage{xcolor} % to access the named colour LightGray
\definecolor{LightGray}{gray}{0.9}
%\usepackage{minted}
\usepackage[autostyle]{csquotes}
\usepackage{longtable}
\usepackage{booktabs}
\usepackage{tablefootnote}
\usepackage{multirow}
\usepackage{adjustbox}
\usepackage{enumitem}
\usepackage{siunitx}
\usepackage{fancyvrb}
\usepackage{soul}
\usepackage{textcomp}
\usepackage{tabularx}
\newlength\someheight
\setlength\someheight{3cm}

\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=1.14}
\definecolor{storeClusterComponent}{HTML}{808080}
\definecolor{dbscan}{HTML}{BEBEBE}
\definecolor{constructCluster}{HTML}{DCDCDC}
\usepackage{tikz} 
\usepackage{subcaption}
% \usetikzlibrary{shapes.geometric}
\usetikzlibrary{shapes,calc,shadows,arrows}
\usepackage{pgf-pie}
\usepackage{etoolbox}
\newtoggle{showpct}
\usepackage{xcolor,colortbl}


\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}
\usepackage[most]{tcolorbox}
%\usepackage{minted}

\newtcbtheorem{Summary}{\bfseries Summary}{enhanced,drop shadow={black!50!white},
  coltitle=black,
  top=0.3in,
  attach boxed title to top left=
  {xshift=1.5em,yshift=-\tcboxedtitleheight/2},
  boxed title style={size=small,colback=pink}
}{summary}


\newtcolorbox[auto counter]{summary}[1][]{title={\bfseries Summary~\thetcbcounter},enhanced,drop shadow={black!50!white},
  coltitle=black,
  top=0.3in,
  attach boxed title to top left=
  {xshift=1.5em,yshift=-\tcboxedtitleheight/2},
  boxed title style={size=small,colback=pink},#1}

\usepackage[round]{natbib}


\usepackage{etoolbox}
% \usepackage[hyphens]{url}
% \usepackage{hyperref}
% \PassOptionsToPackage{hyphens}{url}
% \hypersetup{colorlinks,
%     citecolor=blue, 
%     urlcolor=black,
%     linkcolor=blue}
% \newcommand*{\escape}[1]{\texttt{\textbackslash#1}}
% \newcommand*\circled[1]{\tikz[baseline=(char.base)]{
%             \node[shape=circle,draw,inner sep=1pt] (char) {#1};}}
\makeatletter
\patchcmd{\pgfpie@slice}%
{\scalefont{#3}\beforenumber#3\afternumber}%
{\iftoggle{showpct}{\scalefont{#3}\beforenumber#3\afternumber}{}}%
{}{}

% Patch case where name and year are separated by aysep
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

% Patch case where name and year are separated by opening bracket
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\def\srcfile[#1,#2]#3{
    \node [draw, fill=white, minimum height=1.7cm, minimum width=1.35cm, rounded corners, double copy shadow={shadow xshift=0.1cm, shadow yshift=0.1cm}] (#1) at #2 {};
    \node[align=center, font=\sffamily\fontsize{5}{1.5}\selectfont] at #2 {#3};
}

\makeatother

\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}
\definecolor{dgreen}{rgb}{0.0, 0.5, 0.0}

%\renewcommand{\lstlistingname}{Figure}
\lstset{
    frame=single,
    tabsize=4,
    showstringspaces=false,
    columns=flexible,
    basicstyle={\small\ttfamily},
    keywordstyle=\color{blue},
    commentstyle=\color{dkgreen},
    stringstyle=\color{mauve},
    breaklines=true,
    breakatwhitespace=true,
    escapeinside={<@}{@>},
}

\usepackage{mdframed}
\newcounter{finding}
\newmdenv[%
    linewidth=0.6pt,
    linecolor=black,
    outerlinewidth=0pt,
    skipabove=0pt,
    skipbelow=0pt,
    settings={\global\refstepcounter{finding}},
]{myfinding}

\newcommand{\finding}[1]{
    \vspace{0.5em}
    \begin{myfinding}
    % \vspace{0.25em}
	\textbf{\textit{Finding~\arabic{finding}}}: #1
 	% \vspace{-0.25em}
    \end{myfinding}
    \vspace{0.5em}
}


\newcommand{\yiming}[1]{\textcolor{violet}{{\it [Yiming says: #1]}}}
\newcommand{\haonan}[1]{\textcolor{dkgreen}{{\it [Haonan says: #1]}}}
\newcommand{\maxime}[1]{\textcolor{red}{{\it [Max says: #1]}}}
\newcommand{\heng}[1]{\textcolor{blue}{{\it [Heng says: #1]}}}

\newcommand{\hadoop}{\href{https://github.com/apache/hadoop}{\javainline{Hadoop}}}
\newcommand{\hadoopO}{\href{http://hadoop.apache.org}{\javainline{Hadoop}}}
\newcommand{\jboss}{\href{http://www.jboss.org/jbossas}{\javainline{JBoss}}}
\newcommand{\hbase}{\href{https://github.com/apache/hbase}{\javainline{Hbase}}}
\newcommand{\hive}{\href{https://github.com/apache/hive}{\javainline{Hive}}}
\newcommand{\zookeeper}{\href{https://github.com/apache/zookeeper}{\javainline{Zookeeper}}}
\newcommand{\tomcat}{\href{https://github.com/apache/tomcat}{\javainline{Tomcat}}}
\newcommand{\lucene}{\href{https://github.com/apache/lucene-solr}{\javainline{Lucene-solr}}}
\newcommand{\actvieMQ}{\href{https://github.com/apache/activemq}{\javainline{ActiveMQ}}}
\newcommand{\maven}{\href{https://github.com/apache/maven}{\javainline{Maven}}}
\newcommand{\ant}{\href{https://github.com/apache/ant}{\javainline{Ant}}}
\newcommand{\empireDB}{\href{https://github.com/apache/empire-db}{\javainline{Empire-DB}}}
\newcommand{\karaf}{\href{https://github.com/apache/karaf}{\javainline{Karaf}}}
\newcommand{\logfj}{\href{https://github.com/apache/log4j}{\javainline{Log4j}}}
\newcommand{\mahout}{\href{https://github.com/apache/mahout}{\javainline{Mahout}}}
\newcommand{\mina}{\href{https://github.com/apache/mina}{\javainline{Mina}}}
\newcommand{\pig}{\href{https://github.com/apache/pig}{\javainline{Pig}}}
\newcommand{\pivot}{\href{https://github.com/apache/pivot}{\javainline{Pivot}}}
\newcommand{\struts}{\href{https://github.com/apache/struts}{\javainline{Struts}}}
\newcommand{\openmts}{\href{https://github.com/apache/openmeetings}{\javainline{Openmeetings}}}
\newcommand{\fop}{\href{https://github.com/apache/xmlgraphics-fop}{\javainline{Fop}}}
\newcommand{\jmeter}{\href{https://github.com/apache/jmeter}{\javainline{Jmeter}}}
\newcommand{\rat}{\href{https://github.com/apache/creadur-rat}{\javainline{Rat}}}
\newcommand{\gitpython}{\href{https://github.com/gitpython-developers/gitpython}{\javainline{GitPython}}}
\newcommand{\srcML}{\href{https://www.srcml.org/}{\javainline{srcML}}}

%Command to strikeout text with citations and references
\newcommand{\strikeit}[1]{%
  \ifcorrectingmode
  \mbox{\sout{#1}}%
%  \makebox[\textwidth][s]{\sout{#1}}%
  \fi
}

%********** Minted **********
\makeatletter
\newcommand\notsotiny{\@setfontsize\notsotiny\@vipt\@viipt}
\makeatother

\usepackage[draft=false]{minted}
\newminted{diff}{
    % numbersep=4pt,
    % linenos,
    fontsize=\scriptsize,
	autogobble=true,
	% style=bw,
% 	breaklines=true,
% 	breakafter=.,
% 	breakautoindent,
%     tabsize=2,
%     breakbytoken=true,
%     resetmargins=true
}
\newmintinline{cpp}{}
\newminted{python}{}
\newmintinline{python}{}
% \newminted{java}{}
% \newmintinline{java}{}
%%%%%%%%%%%%%%% java in stream
\newminted{java}{
	fontsize=\small,
	autogobble=true,
	% style=bw,
	breaklines=true,
	breakafter=.,
	breakautoindent,
    tabsize=2,
    % linenos=true,
    breakbytoken=true,
    resetmargins=true}
\newmintinline{java}{
	% style=bw,
    fontsize=\small}
\setminted{%
    style=trac,
    autogobble=true,
    breaklines=true,
    breakafter=.,
    breakautoindent,
    escapeinside=||}
\newcommand{\textjavainline}[1]{\ensuremath\text{\javainline{#1}}}
\DeclareCaptionSubType{listing}
\newcommand{\ji}[1]{\javainline{#1}}

\let\proof\relax
\let\endproof\relax
\let\example\relax
\let\endexample\relax
\usepackage{amsthm}

\theoremstyle{definition}
\newtheorem{dfn}{Definition}

\usepackage{threeparttable}

\usepackage{array}
\definecolor{dodgerblue}{RGB}{30,144,255}
\definecolor{orange}{RGB}{255, 120, 8}

\newcommand{\lstbg}[3][0pt]{{\fboxsep#1\colorbox{#2}{\strut #3}}}
\lstdefinelanguage{diff}{
  basicstyle=\ttfamily\small,
  morecomment=[f][\lstbg{red!20}]-,
  morecomment=[f][\lstbg{green!20}]+,
  morecomment=[f][\textit]{@@},
  %morecomment=[f][\textit]{---},
  %morecomment=[f][\textit]{+++},
}

\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}

% \usepackage[skins]{tcolorbox}
\tcbset{commonstyle/.style={boxrule=0pt,sharp corners,enhanced jigsaw,nobeforeafter,boxsep=0pt,left=\fboxsep,right=\fboxsep}}
\newtcolorbox{mycolorbox}[1][]{commonstyle,#1}

\newcommand{\wrapcolorbox}[2][]{%
  \colorbox{#1}{\tiny \parbox{\dimexpr\linewidth-2\fboxsep}{#2}}
}

\newcommand{\responsecolorbox}[2][]{%
  \colorbox{#1}{\small \textit{\parbox{\dimexpr\linewidth-2\fboxsep}{#2}}}
}

\newcommand{\findcolorbox}[2][]{%
  \vspace{-0.15cm}
  \colorbox{#1}{\normalsize \parbox{\dimexpr\linewidth-2\fboxsep}{#2}}
%   \vspace{0.1cm}
}

% \newcommand{\inlinecode}[2]{\lstinline[language=#1]$#2$}
\def\inline{\lstinline[basicstyle=\ttfamily \scriptsize]}


\usepackage{svg}


% patch \maketitle:
\usepackage{etoolbox}
\newcommand*{\affaddr}[1]{#1} % No op here. Customize it for different styles.
\newcommand*{\affmark}[1][*]{\textsuperscript{#1}}

% \usepackage[misc]{ifsym}

\usepackage{scalerel}
\usepackage{tikz}
\usetikzlibrary{svg.path}

\definecolor{orcidlogocol}{HTML}{A6CE39}
\tikzset{
  orcidlogo/.pic={
    \fill[orcidlogocol] svg{M256,128c0,70.7-57.3,128-128,128C57.3,256,0,198.7,0,128C0,57.3,57.3,0,128,0C198.7,0,256,57.3,256,128z};
    \fill[white] svg{M86.3,186.2H70.9V79.1h15.4v48.4V186.2z}
                 svg{M108.9,79.1h41.6c39.6,0,57,28.3,57,53.6c0,27.5-21.5,53.6-56.8,53.6h-41.8V79.1z M124.3,172.4h24.5c34.9,0,42.9-26.5,42.9-39.7c0-21.5-13.7-39.7-43.7-39.7h-23.7V172.4z}
                 svg{M88.7,56.8c0,5.5-4.5,10.1-10.1,10.1c-5.6,0-10.1-4.6-10.1-10.1c0-5.6,4.5-10.1,10.1-10.1C84.2,46.7,88.7,51.3,88.7,56.8z};
  }
}

\newcommand\orcidicon[1]{\href{https://orcid.org/#1}{\mbox{\scalerel*{
\begin{tikzpicture}[yscale=-1,transform shape]
\pic{orcidlogo};
\end{tikzpicture}
}{|}}}}



\usepackage{listings}
\usepackage{xcolor} % For customizing colors (optional but recommended)

% Define Python-specific settings for listings
\lstdefinestyle{python}{
    language=Python,
    basicstyle=\ttfamily\small,
    keywordstyle=\color{blue}\bfseries,
    commentstyle=\color{green!50!black}\itshape,
    stringstyle=\color{red},
    showstringspaces=false,
    frame=single,
    numbers=left,
    numberstyle=\tiny\color{gray},
    stepnumber=1,
    numbersep=5pt,
    breaklines=true,
    breakatwhitespace=true,
    tabsize=4,
    captionpos=b
}

% Default style for listings
\lstset{style=python}

\usepackage{hyperref}
% \usepackage[hidelinks]{hyperref}



==> 10_Conclusion_and_Future_work.tex <==
\textcolor{blue}{This paper introduces a comprehensive empirical study focused on understanding the trends, topics, and challenges in logging practices discussed by developers on Stack Overflow (SO). Our findings show that questions about logging frequently involve programming concepts and framework/library. Leveraging advanced LLM techniques, we have categorized the discussions into 11 distinct topics. Notably, the three predominant topics—\textit{``Logging Levels and Output," ``General Logging Practices,"} and \textit{``Error Handling and Debugging"}—accounting for 70\% of all discussions.}


\textcolor{blue}{In addition, we observe that \textit{Logging in Containerized Environments} emerged as the most difficult topic, with 64.91\% of its questions lacking accepted answers and a long median resolution time.}

\textcolor{blue}{From our quantitative and qualitative analyses, we have distilled several key insights for various stakeholders, such as effort needed to support logging in containerized environments. Moving forward, we plan to conduct a survey involving industrial developers. This future work aims to complement our empirical findings and validate the observed trends on logging topic depending on the team sizes and experiences; its objective is to quantify perceived difficulty and time-to-fix for the top topics, identify additional technical or other challenges in logging, and refine the guideline provided in this study.}  


% The survey will complement our empirical results by validating observed trends, prioritizing pain points across ecosystems and team sizes, and identifying any important logging areas we may have missed. Its objectives are to quantify perceived difficulty and time-to-fix for the top topics and to use the findings to refine the guidelines provided in this study.

==> 1_Abstract.tex <==
\textbf{Context:} Logging is a crucial practice in software engineering, aiding developers in debugging applications when errors occur. While existing research has explored logging challenges from an academic perspective through literature reviews and source code analysis, a comprehensive study from the practitioners' perspective remains lacking. 

\noindent\textbf{Objective:} This paper aims to bridge this knowledge gap by presenting an in-depth analysis of trends, topics, and challenges in logging based on a dataset of 216,094 posts from Stack Overflow (SO), a popular Q\&A platform for developers. 

\noindent\textcolor{blue}{\textbf{Method:} 
We analyzed longitudinal trends by examining metadata related to users, questions, and tags associated with logging discussions. To identify prevalent discussion topics, we employed a Large Language Model (LLM)–based classification approach, based on a manually validated ground-truth sample. Topic popularity was assessed through average scores and views, while difficulty was measured using three community-driven metrics: the proportion of questions without accepted answers, the proportion of unanswered questions, and the median time to receive an accepted answer.}

\noindent\textcolor{blue}{\textbf{Results:} 
Our analysis identifies 11 distinct topics, with the top three (General Logging Practices, Error Handling and Debugging, and Logging Levels and Output) accounting for over 70\% of all logging-related discussions. Notably, \textit{Logging in Containerized Environments} emerged as the most difficult topic: 64.9\% of its questions lack an accepted answer, and its median resolution time is among the highest. These findings highlight enduring practitioner struggles with logging in Docker or other containerized environments  and the integration of logging pipelines into orchestrators such as Kubernetes and cloud environments.} 

\noindent\textbf{Conclusion:} This study sheds light on the practical challenges of logging and provides actionable insights for developers, framework vendors, researchers, and educators.


\keywords{
Logging practices, Stack Overflow, Empirical study.
}

==> 2_Introduction.tex <==
Logging is a fundamental practice in software engineering, crucial for recording dynamic information during a program's execution. This process supports real-time analysis and postmortem diagnostics, providing essential data for tasks such as failure diagnosis \citep{fu2013contextual}, performance analysis \citep{nagaraj2012structured}, and anomaly detection \citep{fu2009execution}. To facilitate logging, developers often employ specialized libraries such as Log4j and Logback, which are designed to integrate logging statements seamlessly into Java applications. These libraries allow for the definition of log messages that can describe runtime events using both static and dynamic data.

Each log entry is categorized by a verbosity level such as fatal, error, info, or debug to indicate the severity and importance of the event. For example, logs classified as `fatal' are critical and may halt the program after logging, whereas `debug' logs are more verbose and generally used during the development phase for detailed tracing. The choice of verbosity level helps developers manage the trade-off between obtaining comprehensive log data and minimizing performance overhead. In production environments, logging becomes particularly crucial as it may provide the only real-time data available to developers for diagnosing issues affecting end-users. Consequently, the strategic structuring and management of log data, from its generation to its archival, are vital for the effective maintenance and troubleshooting of software systems.

\begin{lstlisting}[language=Java, caption=Java Log4j logging example, label={lst:code1}]
import org.apache.log4j.Logger;
import org.apache.log4j.BasicConfigurator;

public class Log4jExample {
    /* Get actual class name to be printed on */
    static Logger log = Logger.getLogger(Log4jExample.class.getName());

    public static void main(String[] args) {
        // Configure logger
        BasicConfigurator.configure();
        int errorCount = 5; // Example of a dynamic variable
        // Log messages at various levels
        log.info("This is an info message");
        log.debug("This is a debug message");
        log.error("This is an error message with a dynamic variable: " + errorCount);
    }
}
\end{lstlisting}

Listing \ref{lst:code1} presents a Java code snippet that initializes the Log4j library and demonstrates logging at various severity levels. It includes an error message that incorporates a dynamic variable (`errorCount'), illustrating how log messages can be enriched with runtime values to enhance debugging capabilities.

\textcolor{blue}{Over the last decade, researchers have examined logging from multiple angles, including systematic reviews of research trends \citep{gholamian2021comprehensive, rong2017systematic, candido2021log, batoun2024literature}, empirical studies of industrial practices \citep{rong2020can, fu2014developers}, and qualitative investigations of developer perspectives \citep{li2020qualitative}. These studies provide valuable insights: they catalog the benefits and costs of logging, uncover challenges such as balancing log verbosity and overhead, and highlight inconsistencies between developer intentions and the resulting log statements in code.}

\textcolor{blue}{Despite these contributions, significant gaps remain. Systematic literature reviews (SLR) and surveys synthesize knowledge across studies and participants, but they are either limited to the boundaries of prior academic work \citep{gholamian2021comprehensive, rong2017systematic, candido2021log, batoun2024literature} or a relatively small number of practitioners \citep{rong2020can, fu2014developers, li2020qualitative}. Industrial case studies, while rich in context, are typically constrained to a few organizations \citep{rong2020can, fu2014developers}. As a result, we lack a large-scale, cross-cutting view of daily logging challenges developers face across diverse contexts, technologies, and expertise levels.}

\textcolor{blue}{To complement the literature, we explore developers’ perspectives expressed on Q\&A platforms. Stack Overflow (SO)\footnote{\url{https://stackoverflow.com/}}, for example, hosts over 24 million questions and 36 million answers spanning a wide range of technologies, with 29 million registered developers as of August 2025. Investigating logging-related questions posted on Q\&A platforms such as Stack Overflow could reveal logging-related challenges faced by developers in their daily development activities, complementing traditional surveys and interview-based studies.}

% \textcolor{blue}{Many studies exploring the challenges associated with logging practices have primarily relied on surveys of practitioners or reviews of existing literature. For instance, Gholamian et al. \citep{gholamian2021comprehensive} conducted a comprehensive review of the literature, identifying a range of logging challenges and opportunities for the research community—a theme similarly explored by other studies \citep{batoun2024literature, candido2021log, rong2017systematic}. Li et al. \citep{li2020qualitative} surveyed practitioners on the benefits and costs of logging, a method also employed in other research \citep{rong2020can, fu2014developers}.}

% Although surveys of practitioners and literature reviews provide valuable insights, their findings may not fully generalize, as they typically rely on interviews with a limited number of participants and are often grounded in academic publications \citep{peruma2022refactor}. Therefore, there is a need to explore logging challenges faced by practitioners in their real-world development contexts at a large scale. Q\&A platforms like Stack Overflow have become increasingly relevant for addressing these challenging logging questions, offering a rich dataset of real-world problems and solutions.
% As of March 2024, Stack Overflow has over 23 million registered users and hosts more than 24 million questions alongside 35 million answers, providing a comprehensive resource for understanding the dynamics of logging practices across various development scenarios. 

For example, one SO post\footnote{\url{https://stackoverflow.com/questions/2031163}} ask: \textit{``There are different ways to log messages, in order of fatality: FATAL; ERROR; WARN; INFO; DEBUG; TRACE; How do I decide when to use which?; What's a good heuristic to use?"}. This post received an answer within five minutes yet has accumulated over 867K views, suggesting that while the issue may be readily resolved, it continues to attract significant attention. Another example is this post\footnote{\url{https://stackoverflow.com/questions/43937031}} where developers faced issues configuring \textit{``logback"}, a logging framework, and received an accepted answer only after nine months despite being viewed over 25K by other developers; it may indicate that the problem encountered by this developer is difficult to solve.    

\textcolor{blue}{While we acknowledge the limitations of Stack Overflow, such as the absence of demographic metadata, its breadth and openness provide a valuable complement to prior work. Surveys, interviews, and systematic literature reviews (SLRs) can offer this contextual richness but are typically constrained by small sample sizes.}
\textcolor{blue}{By contrast, Stack Overflow provides an unparalleled scale and diversity of reported issues, capturing recurring problems across technologies and contexts. Although we cannot stratify results by demographics, we complement prior literature reviews, surveys, and case studies by systematically mapping the challenges developers articulate in practice, thereby revealing both overlaps with and gaps in existing research. To this end, this paper conducts a comprehensive empirical study of 216,094 logging-related posts on SO to address the following Research Questions (RQs):}

% In light of these observations, we believe that an analysis of logging discussions on SO can provide the research community and stakeholders with a deeper understanding of developers' concerns, thus shedding light on critical logging issues that are most pertinent to developers, to inform research efforts to address them. To this end, this paper conducts a comprehensive empirical study of 75,518 logging-related posts on SO to address the following Research Questions (RQs):

\noindent\hspace*{2mm} \textbf{RQ1 (Trend): How have logging discussions on Stack Overflow grown over the years?} \textcolor{blue}{This research question aims to comprehensively understand the global trends and technological contexts within which logging-related discussions occur on Stack Overflow. We analyzed a dataset comprising 216,094 logging-related questions, 118,196 responses, 146,840 distinct users, and 20,758 associated tags, collected from the Stack Exchange Data Dump \footnote{\url{https://archive.org/details/stackexchange}} by filtering for posts explicitly tagged with ``log", those containing the term in the post title, or those tagged with a specific logging library. Our findings indicate that developers have relied heavily on SO to resolve logging issues, although participation patterns show that most users contribute only once, with limited sustained expertise across discussions.  
When compared with prior studies, logging discussions resemble Continuous Integration (CI) and refactoring in their fragmented engagement.
In terms of technological context, logging stands out as a cross-disciplinary topic. Through manual review of a significant sample of tags, we found that the majority of associated tags were related to \textit{programming concepts} (e.g., \textit{int}, \textit{exception}, \textit{biginteger}) and \textit{frameworks/libraries} (e.g., \textit{Symfony}, \textit{JavaFX}, \textit{Vue.js}), highlighting its foundational role in software engineering. Unlike CI, where tags are dominated by platforms and servers, and unlike refactoring, where tags center on languages and algorithms, logging discussions are spread across multiple dimensions--tools, platforms, frameworks, and concepts. Notably, emerging domains such as machine learning (ML) (\textit{data-science}, \textit{text-classification}) and security (\textit{security}, \textit{protected}, \textit{credential-manager}) increasingly appear in logging contexts, reflecting the growing importance of observability and trustworthy system design.}  
\\
% This research question aims to comprehensively understand the global trends and technological contexts within which logging-related discussions occur on Stack Overflow. We specifically investigate the volume, growth patterns in the number of users involved and questions asked, and the evolution of associated technologies over time. Specifically, we analyze a dataset comprising 75,518 questions, their 62,851 responses, the 59,243 users who participated in these discussions, and the 10,587 tags associated with the logging questions. Our results indicate a high reliance on SO by developers seeking assistance for logging issues. Furthermore, we observed an increasing interest in some associated tags over the years. Most notably, the tags associated with these logging questions predominantly pertain to programming concepts (e.g., \textit{int}, \textit{exception}, \textit{biginteger}, etc) and Framework/Library (e.g., \textit{symfony}, \textit{JavaFX}, \textit{vuejs}, \textit{etc}), reflecting the deep integration of logging practices within software development paradigms. We also observed the appearance of concepts such as machine learning (e.g., \textit{data-science}, \textit{text-classification}, \textit{etc.}) and security (e.g., \textit{security}, \textit{protected}, \textit{credential-manager}, etc.) associated with logging.
\hspace*{2mm} \textbf{RQ2 (Topic): What topics are discussed around logging?} \textcolor{blue}{The goal of this research question is to identify the key topics that developers discuss on Stack Overflow related to logging, as well as to determine their relative frequency. To achieve this, we employed an LLM-based classification approach, grounded in a manually validated ground-truth sample. Our analysis reveals 11 distinct topics, with \textit{General Logging Practices (36.53\%)}, \textit{Error Handling and Debugging (21.27\%)}, and \textit{Logging Levels and Output (14.54\%)} accounting for more than 70\% of all logging discussions. Other specialized topics, such as \textit{Data and TensorBoard Logging (2.56\%)}, \textit{Logging in Containerized Environments (2.36\%)}, and \textit{Testing and CI Pipelines (0.71\%)}, represent smaller but significant areas of practitioner concern.\\}
\hspace*{2mm} \textbf{RQ3 (Challenges): Which topics are the most popular and difficult among logging questions?} \textcolor{blue}{We leverage information from SO to identify the most popular and challenging topics in logging. To assess topic popularity and difficulty, we measured average scores and views as indicators of community attention, and difficulty through three established metrics: the proportion of questions without accepted answers, the proportion of unanswered questions, and the median time to receive an accepted answer. Our findings highlight sharp contrasts across topics. Logging in \textit{Containerized Environments} emerges as the most challenging, with 64.9\% of its questions lacking accepted answers and one of the highest median resolution times. These results underscore enduring struggles with the integration of logging into orchestrators such as Kubernetes, Docker, and cloud platforms. By contrast, \textit{General Logging Practices}--which covers fundamental concerns such as when, where, and how to insert log statements across different programming languages and frameworks--appears among the least difficult (51.56\% without accepted answers) and is resolved most quickly (median 21.36 hours). Similarly, \textit{Logging Levels and Output}--which deals with selecting appropriate severity levels (DEBUG, INFO, WARN, ERROR) and composing meaningful log messages--stands out as both highly popular and relatively easy to resolve. At the other end of the spectrum, \textit{Data and TensorBoard Logging}, which concerns logging in data-intensive systems, while among the least popular topics, still exhibits a high proportion of unresolved questions (59.06\%). Compared to related domains (Continuous Integration and Refactoring), logging emerges as the most difficult and time-consuming, with 56.49\% of questions lacking accepted answers and a median resolution time of 45.37 hours \citep{ouni2023empirical, peruma2022refactor}.}

% reflecting the immaturity of logging practices in machine learning--intensive systems.
% Our analysis indicates that questions related to \textit{Logging in Containerized Environments} are both the most viewed and scored, and they also present the greatest difficulty, as measured by the percentage of questions without accepted answers. Conversely, \textit{General Logging Practices} are less challenging but still maintain considerable popularity. Additionally, topics under \textit{Data and Tensorboard Logging} required the longest time to receive accepted answers.
\noindent The primary contributions of this study are summarized as follows:
\begin{itemize}
    \item We conduct a comprehensive empirical study (mining and analyzing 216,094 SO posts related to logging) aiming to deepen the understanding of challenges, trends, and topics related to logging. %within this domain.
    \item We employ a mixed-method approach, incorporating both quantitative and qualitative analyses, to elucidate the characteristics of logging-related topics and the utilization of logging frameworks.
    \item We compare our findings with related empirical studies on Continuous Integration (CI) \citep{ouni2023empirical} and Refactoring \citep{peruma2022refactor}, highlighting both similarities and differences across domains to position logging within the broader SE research landscape.
    \item We offer practical insights for researchers, developers, tool builders, and educators based on our findings.
    \item We provide a publicly accessible replication package \citep{replication}, which includes the dataset and scripts necessary for replicating our results.
\end{itemize}

The structure of this paper is as follows: Section \ref{sec:approach} outlines our research methodology. Section \ref{sec:result} presents our results and findings. Section \ref{sec: discussion_implication} discusses the implications of our study. Section \ref{sec:related_work} reviews related work. Section \ref{sec:threats_to_validity} addresses potential threats to validity. Finally, Section \ref{sec:conclusion} concludes the paper.

==> 3_Background.tex <==
This section introduces key concepts essential for understanding the work outlined in the paper.

\subsection{Audit in machine learning}
Audit in machine learning involves a systematic examination and evaluation of the performance and behavior of machine learning algorithms and models, to ensure that they are operating as intended, without bias or unintended consequences \citep{Censius2023AIAudit}. This evaluation is typically performed to examine the inputs, outputs, and decision-making process of the algorithm or model, as well as the quality and appropriateness of the data used to train the model. The purpose of the audit is to ensure that the machine learning system is reliable, accurate, fair, and transparent \citep{clark2018machine}. The audit process may involve various techniques and tools, including monitoring, testing, and validation, and it may cover various aspects of the machine learning system, such as data privacy, model interpretability, fairness, and security \citep{clark2018machine, yang2024robustness}. The audit results may be used to identify and mitigate any issues or risks associated with the machine learning system, as well as to improve its performance and usability. Based on the above, the key motivation for our research is to investigate how practitioners monitor responsible AI-related metrics that could be leveraged for auditing compliance with responsible AI principles.
% \heng{Would be good to discuss this work's relation with the audit notion in machine learning, for example, we investigate how practitioners measure responsible AI-related metrics that could be leveraged for auditing compliance to responsible AI principles}

\subsection{Auditing techniques}
In the area of information technology (IT), the audit is the process of evaluating the effectiveness, efficiency, and security of an organization's information systems \citep{otero2018information}. IT audit plays a crucial role in ensuring that organizations' information systems are operating effectively, efficiently, and securely to achieve the desired goals.
To assess the effectiveness of an organization's information systems, IT auditors use various techniques and tools. Some commonly used techniques include:
\begin{itemize}[leftmargin=0.8 pt,align=left]
    \item \textbf{Risk-based auditing}: This technique involves identifying the most significant risks to an organization's information systems and directing the audit effort towards those areas. By prioritizing their work, auditors ensure that they focus on the most critical aspects of the system.\citep{griffiths2012risk}.
    \item \textbf{Compliance auditing}: This technique involves assessing the organization's compliance with laws, regulations, and industry standards. Compliance auditing is essential to ensure that organizations meet legal, regulatory requirements, and certification standards \citep{thottoli2021relevance}. 
    \item \textbf{Process-based auditing}: This technique involves evaluating the organization's processes to ensure they are efficient, effective, and meet business objectives. Process-based auditing helps auditors to identify areas for improvement and recommend process changes to improve the overall effectiveness of the system \citep{guldenmund2006development}.
\end{itemize}
ML auditing requires a tailored set of techniques and tools since it has its unique challenges and more specific auditing requirements, such as the need for explainability and transparency of the decision-making process and the need for monitoring the data and algorithmic bias.
% \heng{Discuss how this work relate to the auditing techniques, e.g., belong to which technique, or why ML auditing is different from these techniques}

\subsection{Continuous auditing}
Continuous auditing (CA) and continuous monitoring (CM) represent integral components of a robust framework for ensuring responsible AI practices. Continuous auditing, as detailed in the Global Technology Audit Guide (GTAG), is an ongoing process of risk and control assessments facilitated by advanced technology. It transitions from periodic to continuous evaluations, encompassing a wide spectrum of transactions and data sources, such as security levels, logging incidents, and changes in IT configurations \citep{gtag}. This methodology allows internal audit functions to offer real-time assurance on effective risk management and control frameworks, substantially enhancing efficiency and providing deeper insights.

Continuous monitoring, stands as a cornerstone for management, enabling an uninterrupted assessment of control effectiveness and risk identification within business processes. It aims to refine business activities in alignment with ethical and compliance standards, fostering more informed risk-related decisions. When harmonized, CA/CM bolsters an organization's capability to identify and address issues in real-time, thus promoting a culture of transparency and accountability essential in the context of responsible AI applications \citep{gtag}.

Integrating continuous auditing into the development and oversight of AI applications, especially in logging metrics related to responsible AI principles like fairness, transparency, and accountability, is crucial. By continuously auditing AI systems for adherence to these principles, organizations can detect and mitigate ethical and operational risks more effectively \citep{deloitecacm}. This approach not only aligns with the increasing regulatory and societal demands for ethical AI but also supports the sustainable integration of AI technologies into business processes \citep{deloitecacm}. Moreover, it facilitates the provision of continuous assurance to stakeholders that AI applications operate within established ethical frameworks, thereby fostering trust and ensuring the long-term viability of AI initiatives.


\subsection{Responsible AI/ML principles}
\label{sec:resp}
Responsible AI/ML refers to the ethical and responsible development, deployment, and use of artificial intelligence and machine learning technologies \citep{deshpande2022responsible}. The growing adoption of AI/ML in various domains has raised concerns about their impact on society, including issues related to fairness, privacy, security, transparency, accountability, and explainability \citep{de2021companies}. Responsible AI/ML seeks to address these concerns and ensure that AI/ML technologies are developed and used in a way that is safe, ethical, and trustworthy. 
Responsible AI/ML involves several key principles, including fairness, accountability, transparency, privacy, and security \citep{de2021companies}.
% \heng{Would be good to use a list to precisely define the principles that are considered in this paper}
\begin{itemize}
    \item \textbf{Fairness}: requires that AI/ML applications do not discriminate against any individual or group based on race, gender, age, or other factors.
    \item \textbf{Accountability}: refers to the responsibility of developers and users of AI/ML applications to ensure that they are used responsibly and ethically. 
    \item \textbf{Transparency \& Explainability}: requires that AI/ML applications be understandable and interpretable and that their decision-making processes can be explained to stakeholders.
    \item \textcolor{blue}{\textbf{Interpretability}: emphasizes the ability to understand and articulate how an AI/ML model generates its predictions or outputs, ensuring that its operations can be traced and justified.}
    \item \textbf{Privacy}: requires that AI/ML applications protect the confidentiality of personal data and do not violate individuals' privacy rights.
    \item \textbf{Security \& Safety}: requires that AI/ML applications are secure and resistant to attacks or malicious use. 
\end{itemize}
   

Many organizations are now advocating for responsible AI; this is the case of the European Union (EU) which published a General Data Protection Regulation (GDPR) in 2018 to regulate the processing of personal data within the EU. This regulation includes provisions that require organizations to ensure that automated decision-making processes, including those based on AI, are transparent, explainable, and fair \citep{voigt2017eu, AIActEU2023}. The IEEE Global Initiative on Ethics of Autonomous and Intelligent Systems and the European Commission's AI have developed a set of guidelines to support the ethical design and deployment of autonomous and intelligent systems\citep{chatila2019ieee, neuwirth2022eu}. These guidelines include principles such as transparency, accountability, and privacy, and aim to promote the responsible use of AI \citep{chatila2019ieee, AIActEU2023}. In 2018, the Montreal Declaration for Responsible AI was also published to provide guidelines for the responsible development and deployment of AI. The Montreal Declaration includes principles such as transparency, accountability, and the protection of privacy and human dignity \citep{MontrealDeclaration2023}. 

However, implementing and ensuring adherence to these principles presents significant challenges. Without effective auditing mechanisms, operationalizing and enforcing these principles can be difficult. Our research aims to bridge this gap by investigating how metrics aligned with responsible AI principles are documented and utilized. Through this work, we aspire to contribute to the development of AI/ML technologies that not only advance in capability but also in their contribution to a just and ethical digital society.

\subsection{Responsible AI/ML library}
\label{sec:respon}
Responsible AI libraries serve as comprehensive frameworks or sets of functionalities that allow developers, researchers, and data scientists to assess, improve, and guarantee the ethical deployment of AI technologies. These libraries are grounded in the recognition that ensuring the responsible use of AI transcends mere compliance with existing legal frameworks; it involves a proactive engagement with the ethical dimensions of technology development.

The landscape of these tools is diverse, reflecting the multifaceted challenges of operationalizing responsible AI principles. From AIF360 to SHAP and OPACUS, each library offers unique approaches to diagnose, mitigate, and elucidate biases across different stages of ML model development from data collection and preprocessing to model training and evaluation. This variety not only accommodates the specific needs and contexts of different AI projects but also enriches the toolkit available to practitioners aiming to uphold ethical standards in their work.

These libraries offer feature model-agnostic capabilities, underscoring the universal applicability of responsible AI practices across various model architectures and applications. By providing metrics for fairness analysis, explanations for model decisions, and mechanisms for data privacy and security, these tools embody a practical response to the global call for ethical consideration in AI projects. 

In summary, responsible AI libraries are instrumental in bridging the gap between abstract ethical principles and concrete technical practices. They offer the means to operationalize responsible AI principles effectively, ensuring that AI and ML technologies are developed and deployed in ways that are not only innovative and efficient but also ethical and equitable. As such, these libraries play a pivotal role in the ongoing journey towards responsible AI, embodying the collective effort of the tech community to foster AI systems that are trustworthy, reliable, and aligned with human values.


==> 4_Approach.tex <==
To explore logging practices and their evolution on Stack Overflow, we adopted a mixed-methods approach combining qualitative and quantitative analyses similar to methodologies used in prior studies ~\citep{gujral2018empirical,openja2020analysis,wen2021empirical,yahmed2023deploying,ouni2023empirical}. This approach focuses on collecting and analyzing posts from Stack Overflow that are relevant to logging. Our methodology, which is clearly illustrated in Figure 2, consists of two main steps: (1) extraction of logging posts, and (2) analysis of these posts.
\subsection{Extracting logging posts}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{ML_logging_overview-cropped.pdf}
    \caption{Overview of our methodology}
    \label{fig:methodology}
\end{figure}
\begin{itemize}[leftmargin=0.8 pt,align=left]
    \item[] \textbf{Stack Overflow Database:} The Stack Overflow dataset was obtained from the Stack Exchange Data Dump on June 6, 2025. This dataset contains posts dating back to July 31, 2008, and each post's metadata includes its identifier, type (e.g., Question, Answer, Wiki), creation date, body, title, score, view count, and up to five tags representing its topics. Notably, Stack Overflow allows the author of a question to validate an answer by marking it as ``accepted'', signifying its effectiveness in addressing the question. In the SO gamification model, users are encouraged to participate actively and provide quality content through a system of rewards and reputation points. Users can vote on the usefulness of posts, with upvotes increasing a post's visibility and the poster's reputation score. High-scoring contributions are more prominently displayed, stimulating users to produce accurate and helpful answers. This system enables a self-regulating community where expertise is recognized and rewarded, promoting an environment rich in professional peer-to-peer engagement and knowledge exchange.
    % \item[] \textbf{Collect relevant logging posts} To extract posts related to logging, we queried the Stack Exchange Data Dump, initially selecting posts tagged with ``logging'' or containing this term in their titles while excluding the body text to avoid false positives, a method aligned with many previous studies \citep{ouni2023empirical, rosen2016mobile, peruma2022refactor}. We extracted 44,738 posts based on tags and 15,000 based on titles. Our initial dataset ($D_0$) comprises 59,767 posts with 10,587 distinct logging tags ($T_0$). Three authors of this paper, each with a minimum of six years of experience in software engineering, artificial intelligence, and cloud computing, manually reviewed $T_0$ to identify specific logging libraries, as some posts may be tagged with a library-specific tag but not include the term ``logging'', e.g., PostID = 74989141\footnote{\url{https://stackoverflow.com/questions/74989141}}. We identified forty different logging libraries, detailed in our replication package \citep{replication}. Incorporating these library tags, we collected a total of 97,209 posts ($D_1$). After merging $D_0$ and $D_1$ and removing duplicates, we compiled a final set of 75,518 unique posts ($D_2$). Our complete dataset is available in our replication package \citep{replication}. Table \ref{tab:collected_data} shows that out of 75,518 posts, 62,851 (83.2\%) received at least one answer, while 34,996 (46.3\%) had an accepted answer.
    % \input{Table/Summary Statistic}

    \textcolor{blue}{\item[] \textbf{Collect relevant logging posts}:
    To extract posts related to logging, we queried the Stack Exchange Data Dump using the stem ``log'' in both the \emph{Title} and \emph{Tags} fields (we excluded bodies to reduce false positives, since titles and tags succinctly convey a question’s primary intent \citep{ouni2023empirical, rosen2016mobile, peruma2022refactor}). This yielded 387{,}412 title matches and 237{,}613 tag matches; after de-duplication our initial corpus was $D_0=\,$432{,}896 unique posts with $T_0=\,$16{,}266 distinct tags.}
    
    \textcolor{blue}{Because broad ``log*'' queries admit many domain-external uses, we applied a reproducible sanitization pipeline to \emph{Title} and \emph{Tags} using a curated set of regular expressions to remove: authentication/login (\texttt{login}, \texttt{logout}, \texttt{authlogic}), UI dialogs (\texttt{*dialog*}, \texttt{messagebox}, etc), mathematics/statistics (\texttt{log-likelihood}, \texttt{logistic-regression}, \texttt{n log n}, \texttt{logsumexp}, \texttt{lognormal}, \texttt{logloss}, \texttt{logspace}, \texttt{logprob}, etc), programming languages/tools (\texttt{prolog}, \texttt{verilog}, \texttt{systemverilog}, \texttt{netlogo}, \texttt{anylogic}, \texttt{logisim}, \texttt{logitech}, \texttt{saleslogix}, etc), VCS commands (\texttt{git log}, \texttt{hg log}, \texttt{svn log}, etc), and tracking (\texttt{worklog}, \texttt{keylogger}, etc). The full list and code are provided in our replication package \citep{replication}. After filtering, the cleaned seed set was $D_0=\,$114{,}678 posts with $T_0=\,$16{,}100 tags}.
    
    \textcolor{blue}{The first three authors of this paper, each with at least six years of experience in software engineering, artificial intelligence, and cloud computing, then manually reviewed $T_0$ to enumerate library-specific logging tags (some posts use library tags without the explicit word ``logging''; e.g., PostID~=~74989141\footnote{\url{https://stackoverflow.com/questions/74989141}}). We identified 40 logging libraries (listed in the replication package) and, by incorporating these tags, collected an additional $D_1=\,$97{,}209 posts.}
    
    \textcolor{blue}{During auditing, we found a small number of posts initially removed by our negative patterns that were in fact about logging (e.g., PostID~=~4370282\footnote{\url{https://stackoverflow.com/questions/4370282}} matches the token \texttt{blog} but discusses logging). For such cases, we applied a whitelist promotion based on the presence of library-specific logging tags in $D_1$ and promoted true positives back into the seed. This increased the cleaned seed from 114{,}678 to 118{,}885 posts; we refer to this promoted seed as our final $D_0$.}
    
    \textcolor{blue}{Finally, we merged the promoted seed $D_0$ with the library-expanded set $D_1$ and removed duplicates, yielding $D_2=\,$216{,}094 unique posts and $T_0 =\,$ 20,758 unique tags. Our complete dataset and scripts are available in the replication package \citep{replication}. Table~\ref{tab:collected_data} summarizes that, of the 216{,}094 posts, 118{,}196 (\textbf{54.7}\%) received at least one answer and 87{,}197 (\textbf{40.4}\%) have an accepted answer.}
    % \input{Table/Summary Statistic}
\begin{table}[htbp]
\centering
\caption{Overview of our collected dataset.}
\label{tab:collected_data}
%\begin{adjustbox}{width=0.8\textwidth}
\begin{tabular}{@{}lr@{}}
\toprule
Metric                             & Value \\ \midrule
Number of posts                  & 216,094 \\
Number of answered posts     & 118,196 \\
Number of accepted answers       & 87,197 \\
Number of distinct tags          & 20,758 \\
Number of distinct users         & 146,840 \\
Average number of tags per question & 3 \\
Average number of answers per question & 1.35 \\ \bottomrule
\end{tabular}
%\end{adjustbox}
\end{table}
    
\end{itemize}

\subsection{Data analysis}
\begin{itemize}[leftmargin=0.8 pt,align=left]
    \item[] \textbf{Step 1. Trend (RQ1):} To assess the trend of logging on SO, we adapted methodologies from prior studies \citep{chen2020comprehensive,gujral2018empirical,openja2020analysis,lopez2018investigation,bagherzadeh2019going,rosen2016mobile,ouni2023empirical}.
    We first analyzed the following metrics: the number of questions, which measures the total number of logging-related queries posted annually, indicating the popularity and community interest over time; the number of questions with accepted answers, assessing the effectiveness of community responses by quantifying how many queries receive satisfactory resolutions each year; the number of questions without accepted answers, highlighting unresolved issues and potential knowledge gaps; and user engagement per year, reflecting the level of community involvement in logging discussions. Collectively, these indicators provide a comprehensive overview of the topic's trends on Stack Overflow \citep{chen2020comprehensive,wen2021empirical}. Subsequently, we analyzed statistics of SO users engaging in logging discussions to identify the subset of users responsible for logging questions and answers. \textcolor{blue}{Finally, we manually analyzed a statistically significant sample of the initial set of tags (T0 = 20,758 tags) to identify the concepts and technologies associated with logging. To ensure the representativeness of our manual review, we selected a sample corresponding to a 99\% confidence level and a 5\% confidence interval. The first two authors independently coded the selected tags, made annotation notes, and then discussed their observations to resolve disagreements and converge on a finalized set of categories. This coding approach, which has been successfully applied in prior empirical studies of developer discussions on SO \citep{peruma2022refactor, ouni2023empirical}, allowed us to construct a taxonomy of concepts or technologies associated with logging. The results of this first step are presented in Section 3.1 to address RQ1.}
    
    
    % Finally, we manually reviewed $T_0$ to understand the concepts or technologies associated with logging. Our analysis covers the period from the first appearance of logging discussions up to April 4, 2025, using data from our dataset $D_2$. The results of the first step are presented in Section \ref{sec:RQ1} to address \textbf{RQ1}.

    
    \item[] \textbf{Step 2. Popular topic (RQ2):} \textcolor{blue}{The goal of this step is to extract prevalent topics from SO discussions related to logging practices. We employed a Large Language Model to assist in the discovery of these topics. Several studies have leveraged LLMs as evaluators or ``judges" in software engineering tasks, such as code generation, summarization, evaluation, and bug detection \citep{tong2024codejudge, he2025code, crupi2025effectiveness}. In this study, we utilize LLMs as a judge for topic discovery, similar to previous work in the field of software engineering \citep{mu2024large, doi2024topic, li2025software}.} 

    \textcolor{blue}{We adopted a reference-based judging approach, as suggested by \citep{lin2024engineering}, which requires ground truth data from real-world sources to assess how well a sample aligns with an ideal response. For our LLM, we chose the GPT-4o-mini model, as it is cost-effective and provides performance comparable to GPT-4, while being more affordable for large-scale use \citep{verdet2023exploring}. We set the temperature parameter to 0, as done in previous studies \citep{verdet2023exploring}, to ensure deterministic and consistent outputs.}
    
    \textcolor{blue}{\textbf{LLM-Based Topic Classification:}
    Using a fixed prompt, we asked the LLM to act as an expert in logging practices and software engineering. This approach optimized the LLM's ability to generate precise responses \citep{wang2024ai}. We prompted the LLM to classify Stack Overflow posts (both the title and body) into predefined logging topics. If no topic matched, the LLM was instructed to propose a new topic. Additionally, for each topic classification, the LLM was asked to extract important keywords to justify its classification, and the results were returned in JSON format.}
    
    \textcolor{blue}{\textbf{Data Preprocessing:}
    Before prompting the LLM, we preprocessed the input (title + body) by removing HTML code, tags, and email addresses to avoid noise and ensure clean data.}
    
    \textcolor{blue}{\textbf{Ground Truth Construction:}
    To build the ground truth sample for topic classification, we manually analyzed 10\% of our $D_2$ dataset. The goal was to identify an initial set of topics for the classification task. The first two authors, both PhD students with over six years of experience in software engineering, collaboratively analyzed the pilot sample through discussions and open coding. Open coding is a popular method used in software engineering to develop taxonomies \citep{verdet2023exploring, abbassi2025unveiling}. 
    During this analysis, the authors read through the titles and bodies of the posts and identified important keywords that could serve as initial topic labels. Without an initial taxonomy of logging topics, inefficient labels were iteratively refined and merged. This process led to the identification of 11 topics, which were used as the ground truth and starting point for classification. To reduce the risk of hallucination by the LLM \citep{sollenberger2024llm4vv}, we provided a brief description of each of the 11 topics in the prompt.}
    
    \textcolor{blue}{\textbf{Topic Classification and Iteration:}
    The LLM was then asked to classify 40\% of the remaining $D_2$ dataset into the 11 predefined topics, and if any posts did not fit, the LLM was instructed to propose new topics. After reviewing the classifications, the first two authors found that new topics proposed by the LLM were too specific to .NET framework logging practices. These posts, associated with the new topics, were reviewed and incorporated into the existing 11 topics, as they shared similarities with posts already classified under those topics, particularly with a topic related to .NET logging, ``NLog and .NET Logging".}
    
    \textcolor{blue}{\textbf{Final Manual Review and Consistency Assessment:}
    In the final step, the first two authors separately labelled the remaining 50\% of the dataset. Once the entire dataset was labeled, we assessed the inter-rater reliability by calculating the Cohen's Kappa score \citep{mchugh2012interrater} to measure the consistency between the two reviewers. We achieved a Kappa score of 0.781, which aligns with the results from previous studies in software engineering \citep{foalem2024studying, abbassi2025unveiling}. All disagreement cases were resolved during meeting discussion.} 
    
    % ### Summary
    % In summary, we used a systematic approach to classify Stack Overflow logging posts into topics, starting with a manually curated set of topics as the ground truth and employing LLMs for topic discovery and classification. Through iterative refinement and inter-rater reliability assessment, we ensured consistent and reliable topic labels for further analysis.
    
    
    
    % This step aims to extract prevalent topics within SO logging discussions. To accomplish this, we employed Latent Dirichlet Allocation (LDA) \citep{blei2003latent}, a state-of-the-art, widely adopted unsupervised machine learning technique for identifying distinct topics in a large volume of documents \citep{openja2020analysis,peruma2022refactor,rosen2016mobile}. Our approach began with thorough preprocessing of data extracted from SO. Each post's title and body were concatenated to form a single document, which was then cleansed of HTML tags (e.g., \textless p\textgreater \textless /p\textgreater), code snippets (i.e., enclosed in \textless code\textgreater \textless /code\textgreater tags), and irrelevant symbols or non-alphabetical characters such as URLs, special characters, punctuation, numbers, and images. Additionally, we removed stop words (e.g., ``and'', ``a'', ``the'', ``we'') using the NLTK stop word kit and improved text quality by employing bi-grams and uni-grams \citep{tan2002use}. We then applied lemmatization to convert words to their meaningful base forms (i.e., lemmas) \citep{plisson2004rule}. This cleanup was essential to minimize noise and improve the text's relevance for LDA processing. Numerous studies have utilized LDA to identify diverse topics in SO data \citep{peruma2022refactor, ouni2023empirical, rosen2016mobile}. To achieve optimal results with LDA for our logging discussion data, we configure several key parameters based on established methodologies from previous studies. Below is a breakdown of each parameter we adjusted. 
    
    % \textbf{Number of Topics:} We varied the number of topics from 2 to 60. The choice of the number of topics plays a critical role in shaping the granularity of the results, with lower values generating general topics and higher values yielding more specific, albeit potentially noisy, topics. 
    
    % \textbf{Iterations:} We fixed the number of iterations at 100, where each iteration represents a complete pass through the entire dataset, as previous studies \citep{peruma2022refactor, ouni2023empirical} show that using 100 iterations is sufficient for similar contexts. The iteration count is crucial for model convergence, ensuring that the algorithm adequately adjusts the topic probabilities until stable topic distributions are achieved. 
    
    % \textbf{Passes:} We set the passes at 10, as recommended by \citep{peruma2022refactor}, reflecting the total number of complete passes the learning model makes over the entire dataset. 
    
    % \textbf{Chunk Size:} We selected a chunk size of 500  following the guidelines from the previous studies \citep{peruma2022refactor, ouni2023empirical}. The chunk size dictates the number of documents processed in one batch during training. This setting balances between training speed and model accuracy by determining the volume of data the model analyzes before updating its internal state.
    
    %  We employed coherence scores and perplexity as metrics to fine-tune our model, achieving a peak coherence of 0.39 and a minimum perplexity of -9.01. These values align with those reported in similar studies \citep{peruma2022refactor, ouni2023empirical}, indicating reliable model performance. Specifically, a higher coherence score suggests good topic separation and semantic interpretability, while a lower perplexity score suggests a better predictive performance of the model. This combination of metrics confirms the quality and reliability of the topics extracted from the data \citep{peruma2022refactor}. These metrics guided us in optimizing the model's settings, resulting in the identification of 11 distinct topics.  After conducting the computational modeling using the LDA algorithm, we undertook a rigorous manual topic labeling process to ensure the relevance and interpretability of the extracted topics. Two researchers, both with strong backgrounds in software engineering and artificial intelligence—independently reviewed the top representative keywords for each topic. The labeling was guided by an analysis of shared terms across topics as well as distinctive keywords unique to each topic, enabling a clear semantic differentiation. Following the independent labeling, a third researcher with a solid background in software engineering acted as a referee to resolve any disagreements. These discrepancies were discussed collectively in a group session until a consensus was reached. To assess the reliability of this methodology, we computed the inter-rater agreement between the two primary annotators, obtaining a Cohen’s Kappa score of 0.71 indicating substantial agreement.  Our final list of logging topics comprises 11 topics and provides answers to our \textbf{RQ2}. Table \ref{tab:topic_distribution} shows the results of our topic labeling. Our implementation of LDA is available in our replication package \citep{replication}.
    \item[] \textbf{Step 3. Challenges (RQ3):} To assess popular and difficult logging topics on SO, we utilize popular metrics from previous studies: (1) view count, and (2) score of logging posts to determine the most popular, high scores obtained for these metrics; the most popular is the logging topic. These metrics are then aggregated by topic, calculating the average score and average view count for all questions within each specific topic. This aggregation provides a comprehensive view of which topics are not only popular but also actively engage the community \citep{rosen2016mobile, alomar2020exploratory, peruma2022refactor}. We further evaluate difficult logging posts by examining questions that lack an ``accepted" answer and by analyzing the median time it takes to receive an accepted answer. This approach allows us to identify not only the most popular topics but also those that pose significant challenges to the community, reflecting both unresolved queries and longer wait times for solutions. Our methodology for identifying challenging topics follows established practices from prior research that analyze domain-specific challenges through Stack Overflow data, ensuring that our findings are grounded in a proven analytical framework \citep{openja2020analysis, peruma2022refactor, ouni2023empirical}. This step 3 helps us to answer our RQ3 discussed in section \ref{sec:RQ3}.

     % \Foutse{it is unclear to me why these two metrics are associated with challenges....i would expect metrics related to time to first answer for example...in any case you need to explain the intuition behind the use of these metrics..they are more related to popularity than difficulty}
\end{itemize}




==> 5_Result.tex <==
This section reports about the results of our investigation into logging evolution on SO. The findings are structured around three key research questions, each aiming to shed light on different aspects of logging. These include the trends in logging discussions over time (RQ1), the primary topics within those discussions (RQ2), and the specific challenges faced by developers related to logging (RQ3). 

% \subsection{RQ1: Trend of Logging}
% \label{sec:RQ1}
% In total, we extracted 216,094 logging related post (vs 27,728 for CI related post and 9,489 for refactoring related post in 2019) from which 18,196 (54.7\%) received at least one
% answer and 87,197 (40.4\%) have an accepted answer for 146,840 distinct developers. While refactoring-related question received highes percentage of accepted question (∼64.41\%), and (∼8.73\%) did not received answer for 7,795 distinct developers. While CI related questions 46.2\% had an accepted answer,36.7\% questions received at least one, but not accepted, answer for 17,992 for distinct developers \citep{peruma2022refactor, ouni2023empirical}.
% \autoref{fig:popularity} illustrates the annual distribution and trends of posts and users involved in these posts, either by asking or responding to questions on SO related to logging.  The data spans from 2008 through 2025 and is categorized into four groups: total questions, users, questions with accepted answers, and questions without accepted answers.

% \textit{Trends of Questions}. The blue bars represent the overall number of questions posted annually, showing a generally increasing trend in the volume of questions, except for a plateau from 2021 to 2025, indicating a growing interest in logging within the SO community and similar growing can be obseved from previous study until 2019 \citep{peruma2022refactor, ouni2023empirical}. The green bars indicate the number of questions where users received satisfactory answers that were marked as accepted. It is noted that there was an increase in accepted answers from 2008 to 2012, which then stabilized until 2020 despite the growing number of questions, and began to decrease from 2021 onward. while similar observation can be done for CI-related post \cite{ouni2023empirical} a grow from 2009 to 2012 then stabilized until 2019. For refactory-related post there is a two years grow from 2009 till 2011 then a drastical decrese untill 2019. Illustrated by the red bars, these questions did not receive an answer deemed satisfactory by the user. We believe that future investigation is required to explain the reason why question without accepted answers start to be near question with accepted answer from year 2021, and furter outnumbered question with accepted answer from 2024. Similar pattern is obsever from paper on refactoring-related post where there number of unaccepted answer outnumbered the question with accepted answer in the last year and near in the 3 years before. the story is completed different for ci-related post where the number of unaccepted answer outnumber the number of accepted answer much earlier 5 years before 2019.   

% \textit{Trends of users}. The orange bars indicate the number of unique users involved in posting questions, which correlates with the trends seen in the total number of questions, reflecting enhanced community activity over the years. In general, there is a slow decrease in both, the total number of questions and user involvement in logging questions from 2021 until the end. This can be attribute to external factor like the apprearence of generative model which performing well in issue faced by developers \cite{zhong2024can,
% da2024chatgpt}\\

\subsection{RQ1: Trend of Logging}
\label{sec:RQ1}

\textcolor{blue}{In total, we extracted 216,094 logging-related posts (compared to 27,728 CI-related posts and 9,489 refactoring-related posts in 2019). Among the logging posts, 18,196 (54.7\%) received at least one answer, and 87,197 (40.4\%) had an accepted answer, contributed by 146,840 distinct developers. By contrast, refactoring-related questions had the highest percentage of accepted answers (∼64.41\%), while 8.73\% of them remained unanswered, involving 7,795 developers. For CI-related questions, 46.2\% had an accepted answer, while 36.7\% received at least one (but not accepted) answer, from 17,992 distinct developers \citep{peruma2022refactor, ouni2023empirical}.}

\textcolor{blue}{\autoref{fig:popularity} illustrates the annual distribution and trends of logging-related posts and user activity on SO, covering the period 2008-2025. The data is categorized into four groups: (1) total questions, (2) unique users, (3) questions with accepted answers, and (4) questions without accepted answers. Below, we analyze the trends for questions and users.}

\textcolor{blue}{\textit{Trends in Questions.}  
The blue bars show the overall number of logging questions posted annually. We observe a steady growth in question volume from 2008 until 2020, after which activity plateaued between 2021 and 2025. This reflects a strong and sustained interest in logging-related issues within the SO community, in line with previous findings up to 2019 \citep{peruma2022refactor, ouni2023empirical}.}  

\textcolor{blue}{The green bars represent questions with accepted answers. From 2008 to 2012, the number of accepted answers increased notably. However, despite continued growth in question volume, the trend stabilized between 2013 and 2020, followed by a decline from 2021 onwards. A similar dynamic was reported for CI-related posts, which grew from 2009 to 2012, then stabilized until 2019 \citep{ouni2023empirical}. For refactoring-related posts, a brief two-year growth was observed from 2009 to 2011, followed by a sharp decline until 2019.}  

\textcolor{blue}{The red bars show questions without accepted answers. Strikingly, from 2021 onward, the number of such questions approached that of questions with accepted answers, and by 2024 it exceeded them. This trend mirrors findings from refactoring-related studies, where unanswered questions eventually outnumbered those with accepted answers in the later years, with a near balance in the preceding three years. In contrast, CI-related posts experienced this imbalance much earlier, with unanswered questions outnumbering accepted ones roughly five years before 2019.  
The rise of unanswered questions suggests that community support is struggling to keep pace with newer or more complex challenges, which can be investigated by future study. Moreover, the broader similarity with trends in CI and refactoring indicates that this is not confined to logging, but reflects systemic shifts in SO usage and discussion dynamics.} 

\textcolor{blue}{\textit{Trends in Users.}  
The orange bars indicate the number of unique users involved in logging discussions, either as askers or responders. User participation follows a trajectory similar to the total number of questions, with steady growth until 2020. From 2021 onward, both question volume and user engagement show a gradual decline. This downturn may be attributed to external factors, which could be investigated by future study, particularly the emergence of generative AI models that are increasingly capable of providing rapid and effective solutions to developer issues \citep{zhong2024can, da2024chatgpt}, or the migration of discussion to alternative platforms (e.g., GitHub Issues, Slack/Discord communities) highlight a redistribution of developer knowledge flows \citep{rong2018logging}.}

\textcolor{blue}{\textit{Trends in Tags.}  
Our dataset contains a total of 20,758 distinct tags. Unsurprisingly, the most frequent tag is ``logging'', which appears in 48,965 questions (7.24\% of the dataset). To better understand the evolution of logging practices, we further examined the top 10 most frequent tags, excluding ``logging'' itself (Table~\ref{tab:popular_tags}). These tags fall into two broad groups: programming languages (Java 4.82\%, Python 2.52\%, C\# 2.18\%, JavaScript 1.72\%, PHP 1.33\%, Android 1.33\%) and logging frameworks (Log4j 2.75\%, Log4j2 1.30\%, Logstash 1.29\%, Logback 1.07\%). Together, these top 10 tags account for 20.31\% of all logging-related questions.}  

\textcolor{blue}{\autoref{fig:tags} illustrates the temporal evolution of these tags on SO between 2008 and 2025. Several distinct patterns emerge. Java is the most dominant tag, peaking around 2015 before experiencing a fluctuating decline, reflecting both its longstanding prominence in enterprise programming language solutions and the gradual shift toward newer logging frameworks. Log4j exhibits two distinct waves: an early rise until 2013, followed by a dip and a second pronounced peak around 2020, after which it declined again. Python shows a more gradual increase, peaking between 2018 and 2020, coinciding with the broader adoption of Python in enterprise systems and data-intensive applications that rely heavily on logging, before tapering off \citep{gonzalez2020state}. C\# and JavaScript follow similar trajectories, with peaks between 2018 and 2021 before declining. PHP and Android peak earlier (2013-2015) and then steadily decline, consistent with the maturation and stabilization of those ecosystems. Among logging-specific frameworks, Log4j2 emerges around 2012, peaks between 2016 and 2017, and then declines. Logback and Logstash both rise after 2010, peak between 2015 and 2017, and subsequently decrease.}  

\textcolor{blue}{Notably, nearly all series show sharp declines in the 2021-2025 window. By 2024-2025, most tags converge toward consistently low counts. This contraction parallels the broader decrease in logging-related questions, accepted answers, and user participation during the same period. The dominance of Java reflects its historical centrality in enterprise logging discussions, but its post-2016 decline was not directly offset by the growth of alternatives such as Log4j2, Logback, or Logstash. The earlier peaks for Android and PHP suggest that logging practices in these ecosystems reached a “steady state” sooner, whereas the later peaks for Python and C\# reflect their increasing importance in enterprise contexts during the late 2010s.}  
  
\textcolor{blue}{These tag dynamics highlight how technological advances, ecosystem maturity, and shifts in programming language adoption shape logging practices. The variability in tag trends indicates that logging discussions on SO are not static but evolve with the rise and fall of programming languages, frameworks, and platforms. Our findings also align with broader adoption of programming language popularity \citep{programming}, suggesting that the growth and decline of logging tags are strongly correlated with the adoption curves of their associated technologies.}
 
\textcolor{blue}{When contrasted with prior empirical studies on Continuous Integration (CI) and refactoring, we observe both similarities and differences. In CI-related discussions, the most popular tags center on CI servers and platforms (e.g., Jenkins, TeamCity, GitLab, Docker). These exhibit lifecycle dynamics: older tools (Hudson, Jenkins) decline while newer cloud-native tools (GitLab, Azure DevOps, Docker) rise \citep{ouni2023empirical}. Refactoring-related tags, by contrast, are dominated by programming languages (Java, C\#, JavaScript, Python, Ruby, PHP), with trends closely aligned to language programming popularity: Ruby and PHP peaked early and declined, while Python and JavaScript rose in the late 2010s \citep{peruma2022refactor}. Logging combines both dynamics: it is simultaneously shaped by the popularity of programming languages (Java, Python, C\#) and the adoption cycles or disruptions of logging frameworks (Log4j, Logback, Logstash). The ``double wave'' observed in Log4j, for example, is a unique phenomenon absent in CI or refactoring, reflecting how external shocks (e.g., critical vulnerabilities) can reignite discussions \citep{10628102}.} 
 
\textcolor{blue}{To further investigate the technologies and concepts associated with logging discussions, we conducted a manual classification of tags. From the full set, we reviewed a statistically significant sample of 645 tags, which provides a 99\% confidence level with a 5\% confidence interval. Two authors independently suggested categories, drawing inspiration from prior classification studies \citep{ouni2023empirical, peruma2022refactor}. Categories were then reconciled and finalized through joint discussion, following the methodology of previous work \citep{ouni2023empirical, peruma2022refactor}.}  

\textcolor{blue}{As a result, we identified ten clusters of tags: \textit{Programming Concepts, Framework/Library, Tool/IDE, Platform/Servers, Other, Database Concepts, Operating Systems (OS), Machine Learning Concepts, DevOps Tools, Programming Languages, and Security Concepts}. This categorization illustrates the diversity of technologies involved in logging discussions and highlights how logging evolves across different computing environments.}

% \textit{Trends of tags.} In total our dataset contain 20,758 distinct tags. Not surppringly, the most occurent tags is "logging" representing 48,965 (7.24\%) question containing "logging" tags.  

% We further investigate trend of top 10 tags present in Table \ref{tab:popular_tags} excluding "logging" tags, since this study focus on logging in order to understand the evolution of logging practice. The top 10 tags are all related to programming language (JAVA 4.82\%, Python 2.52\%, c\# 2.18\%, Javascript 1.72\%, php 1.33\%, android php 1.33\%) and logging framework (log4j 2.75\%, log4j2 1.30\%, logstash 1.29\%, logback 1.07\%). The top 10 popular tags account for 20.31\% of logging related question.
% \autoref{fig:tags} illustrates the evolution in the popularity of various logging-related tags on SO over the period from 2008 to 2025. The most frequent tag is ``java," which exhibits a significant peak around 2015 before experiencing a fluctuating decline, possibly reflecting broader shifts in logging practices or the adoption of specific logging frameworks. Among the other tags, ``log4j'' show two waves and early rise until 2013, a dip and a second pronounced peack around 2020 before declining distinct from most other tags. ``Python'' increase more gradually, peaking around 2018-2020 aligning with the increasing use of these languages in development environments that emphasize extensive logging, then declining.  C\# and javascript have a similar curve peak around 2018-2021 then taper off. php and android peak earlier 2013–2015, followed by steady declines, consisten with maturation of those stacks. Logging framework tools log4j2 emerges in 2012 peaks 2016-2017, then declines. logback and logstash rise around 2010 pick around 2015-2017, then decline. Nearly all series drop in the 2021–2025 window; by 2024–2025 they converge toward low counts. This contraction aligns with fewer questions, fewer accepted answers and user in the same period. The java dominance reflects the long-standing footprint of Java in enterprise logging questions; its decline after ~2016 mirrors the overall drop and does not appear to be replaced one-for-one by log4j2, logback, or logstash. Earlier peaks for android/php suggest those ecosystems reached logging “steady state” sooner; later peaks for python/c\# match their growing enterprise usage in the late 2010s.\\


% Overall, the landscape of logging is dynamically shifting due to technological advancements and the introduction of new frameworks and languages. This variability influences the frequency and nature of logging-related discussions on SO platform. Furthermore, our result of the dynamic growing popularity of tags correlate with the growing adoption of popular programming language \citep{programming}.To further investigate technologies or concepts associated with these logging tags, we manually classified the tags to determine the most popular technologies and concepts used in these discussions. We reviewed a statistically significant sample of 645 tags, which represents a confidence level of 99\% and a confidence interval of 5\%. Two authors reviewed the tags inspiring by previous study category \citep{ouni2023empirical, peruma2022refactor}, each author suggest category, we furtuer compare category and discuss througth meeting on the finally category following previous study approach \citep{ouni2023empirical, peruma2022refactor}. As a result, we categorized the tags into ten clusters: \textit{Programming concepts, Framework/Library, Tool/IDE, Platform/Servers, Other, Database Concepts, Operating System (OS), Machine Learning Concepts, DevOps Tools, Progamming Language, Security Concepts}. This categorization helps illustrate the diversity and evolution within the field of logging across various computing environments. 

\textcolor{blue}{Figure \ref{fig:tags_concepts} shows the distribution of tags associated with logging. The majority of tags are related to programming concepts (40\%), such as ``exceptions" and ``biginteger", etc. Frameworks and libraries are the second most prevalent categories linked to logging (14.9\%), with examples including Symfony, Laravel, and Log4j. Tools and IDEs, such as Pentaho, VSCode, and Eclipse, account for 11.8\% of the tags, indicating their significant role in logging practices. The category Platform/Server (e.g., AWS, Tomcat, Apache, etc) comprises 7.8\% of the tags associated with logging. Database concepts represent 5\% of the tags, featuring items like ``submitchanges" and ``delta-live-tables". Operating systems such as Windows, iOS, and RedHat are linked to 4.2\% of the logging-related tags. Machine learning tools and concepts, including YOLO, Seq2Seq, and data science, contribute to 3.7\% of the tags. DevOps tools such as Git, TeamCity, Docker, and Ansible make up 3.3\% of the category. Popular programming languages like Python, Java, Android, and PHP fall under the Programming Language category, accounting for 2.3\% of the tags. The final category, Security Concepts, includes tags such as \textit{security, protected, and credential-manager}, which comprise 2\% of the distribution. This categorization highlights the diverse technologies and areas that integrate with logging practices across various software development environments.}  \\
\textcolor{blue}{When compared to the distribution of CI and refactoring tags, several differences emerge. In the CI study, the dominant categories were \textit{platforms and servers} (40.15\%) and \textit{concepts} (20.52\%), with relatively fewer tags linked to programming languages (8.5\%) \citep{ouni2023empirical}. This reflects CI’s strong association with server infrastructure (e.g., Jenkins, TeamCity, Docker) and process-oriented concepts (e.g., continuous deployment). In contrast, the refactoring study reported a predominance of \textit{algorithms and programming concepts} (43.22\%) and \textit{framework/library/API} tags (21.61\%), with programming languages (10.26\%) also playing a more substantial role \citep{peruma2022refactor}. Logging occupies a middle ground between these two domains. Like refactoring, it shows a heavy reliance on programming concepts. Unlike CI, where platform/server categories dominate, logging discussions are more evenly distributed across multiple categories, frameworks, IDEs, servers, databases, and even machine learning. This diversity underscores the fact that logging is not confined to infrastructure or language issues alone but cuts across the entire software stack, from low-level programming concepts to emerging fields such as ML and DevOps.} \\  
\textcolor{blue}{The presence of machine learning and security-related tags further indicates that logging is increasingly tied to modern concerns such as AI monitoring \citep{bodor2023machine}, observability \citep{sakinala2025monitoring}, and trustworthy system design \citep{foalem2025logging} dimensions less visible in prior CI and refactoring studies. This diversity highlights the evolving role of logging as both a cross-cutting concern and a foundational practice for emerging domains.}\\
\textcolor{blue}{To understand community engagement in logging discussions on Stack Overflow, we investigated the distribution of users participating in both questioning and answering. We can observe in Table \ref{tab:post_distribution}, that the majority of users (75.99\%) have posted only once, highlighting a trend where many engage primarily to seek answers to specific logging-related questions. This one-time posting behavior is accompanied by a sharp decline in users who post more frequently; only 16.26\% of users have posted twice, and fewer than 4\% have posted three times. This pattern is consistent, with the percentage of users decreasing as the number of posts increases, as presented in \autoref{fig:popularity}. Regarding answers, 76.81\% of users who have their answers accepted have only one accepted answer, suggesting that while many contribute valuable solutions, they do not regularly participate in logging discussions. This trend implies a potential lack of deep, sustained expertise and mentorship within the logging discussion community on SO. Similarly, the percentage of users with non-accepted answers follows a comparable trend, where 80.48\% of users do not receive acceptance for their single contribution. This community engagement observation isn't specific to logging and can also be observed in previous studies \citep{ouni2023empirical, peruma2022refactor}.}


% When contrasted with other domains, some interesting differences emerge. In the CI study, Ouni et al. found that 87.36\% of users asked at most one question, and 88–92\% of answerers contributed only once \citep{ouni2023empirical}. 

% This indicates that CI discussions also suffer from highly fragmented engagement, with many developers appearing on SO only to resolve a single, immediate issue. In contrast, the refactoring study reported slightly more balanced engagement, with stronger representation from frequent contributors, likely reflecting the deeper expertise required for design and restructuring tasks:\citep{peruma2022refactor}.  


% Logging falls closer to CI than to refactoring in terms of participation dynamics: both logging and CI show heavy reliance on one-time contributors and limited sustained expertise. However, a notable distinction is that logging involves a broader intersection of frameworks, languages, and infrastructure (as shown in our tag analysis), which might discourage long-term participation by diluting focus across diverse technologies. By comparison, refactoring tends to draw fewer but more engaged contributors with specialized expertise. This suggests that the logging community on SO may provide breadth of participation but lacks the depth of expertise and mentoring structures that refactoring enjoys, leaving gaps in knowledge continuity for complex logging issues.


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Questions_Users_by_Year_cropped.pdf}
    \caption{Popularity trend of logging post on SO over years.}
    \label{fig:popularity}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{Distribution_of_tags.pdf}
    \caption{Logging tags popularity growth over years.}
    \label{fig:tags}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{tags_distribution_pie_chart.png}
    \caption{Distribution of concepts associated with logging.}
    \label{fig:tags_concepts}
\end{figure}


% \input{Table/Popular_tags}
\begin{table}[htbp]
\centering
\caption{Top-10 most popular tags.}
\label{tab:popular_tags}
%\begin{adjustbox}{width=0.6\textwidth}
\begin{tabular}{@{}lrr@{}}
\toprule
Tag          & Occurrence & Percentage \\ \midrule
% logging      & 48,965     & 7.24\%    \\
java         & 32,640     & 4.82\%     \\
log4j        & 18,647      & 2.75\%     \\
python       & 17,037      & 2.52\%     \\
c\#          & 14,795      & 2.18\%     \\
javascript       & 11,633      & 1.72\%     \\
php      & 9,007      & 1.33\%     \\
android        & 9,002      & 1.33\%     \\
log4j2         & 8,815      & 1.30\%     \\
logstash  & 8,775      & 1.29\%     \\ 
logback  & 7,259      & 1.07\%     \\ \bottomrule
\end{tabular}
%\end{adjustbox}
\end{table}
% \input{Table/Post_Distribution}
% \begin{table}[htbp]
% \centering
% \caption{Distribution of the number of posts created by a user.}
% \label{tab:post_distribution}
% %\begin{adjustbox}{width=0.8\textwidth}
% \begin{tabular}{@{}lrr@{}}
% \toprule
% \textbf{Number of posts created by a user} & \textbf{Count} & \textbf{Percentage} \\ \midrule
% \multicolumn{3}{l}{\textit{Questions - total distinct users: 146,840 }} \\
% 1 & 111,584 & 75.99\% \\
% 2 & 23,871  & 16.26\% \\
% 3 & 5,108 & 3.48\% \\
% 4 & 2,775 & 1.89\% \\
% 5 & 1,186 & 0.81\% \\
% Others & 2,316 & 1.58\% \\ \midrule
% \multicolumn{3}{l}{\textit{Accepted Answers - total distinct users: 68,652}} \\
% 1 & 52,731 & 76.81\% \\
% 2 & 11,284 & 16.44\% \\
% 3 & 2,150 & 3.13\% \\
% 4 & 1,217 & 1.77\% \\
% 5 & 464 & 0.68\% \\
% Others & 806 & 1.17\% \\ \midrule
% \multicolumn{3}{l}{\textit{Non-Accepted Answers - total distinct users: 89,835}} \\
% 1 & 72,299 & 80.48\% \\
% 2 & 13,358 & 14.87\% \\
% 3 & 2,074 & 2.31\% \\
% 4 & 1,103 & 1.23\% \\
% 5 & 419 & 0.47\% \\
% Others & 582 & 0.65\% \\
% \bottomrule
% \end{tabular}
% %\end{adjustbox}
% \end{table}
\begin{table}[htbp]
\centering
\begin{threeparttable}
\caption{Distribution of the number of posts created by a user.\tnote{a}}
\label{tab:post_distribution}
\begin{tabular}{@{}lrr@{}}
\toprule
\textbf{Number of posts created by a user} & \textbf{Count} & \textbf{Percentage}\tnote{b} \\ 
\midrule
\multicolumn{3}{l}{\textit{Questions — total distinct users: 146{,}840\tnote{c}}} \\
1 & 111{,}584 & 75.99\% \\
2 & 23{,}871  & 16.26\% \\
3 & 5{,}108   & 3.48\% \\
4 & 2{,}775   & 1.89\% \\
5 & 1{,}186   & 0.81\% \\
Others\tnote{d} & 2{,}316 & 1.58\% \\ 
\midrule
\multicolumn{3}{l}{\textit{Accepted Answers — total distinct users: 68{,}652\tnote{e}}} \\
1 & 52{,}731 & 76.81\% \\
2 & 11{,}284 & 16.44\% \\
3 & 2{,}150  & 3.13\% \\
4 & 1{,}217  & 1.77\% \\
5 & 464      & 0.68\% \\
Others\tnote{d} & 806 & 1.17\% \\ 
\midrule
\multicolumn{3}{l}{\textit{Non-Accepted Answers — total distinct users: 89{,}835\tnote{f}}} \\
1 & 72{,}299 & 80.48\% \\
2 & 13{,}358 & 14.87\% \\
3 & 2{,}074  & 2.31\% \\
4 & 1{,}103  & 1.23\% \\
5 & 419      & 0.47\% \\
Others\tnote{d} & 582 & 0.65\% \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]\footnotesize
\item[a] The table reports distributions over \emph{distinct users} per role (askers, users with accepted answers, users with non-accepted answers), not counts of posts. 
\item[b] Percentages are computed \emph{within each block} (Questions / Accepted Answers / Non-Accepted Answers) using that block’s “total distinct users” as the denominator.
\item[c] “Questions” counts each distinct user who asked at least one logging-related question and groups them by how many questions they asked.
\item[d] “Others” aggregates users with $\ge 6$ contributions in the corresponding role.
\item[e] “Accepted Answers” counts each distinct user who has at least one answer marked as accepted and groups them by how many \emph{accepted} answers they authored.
\item[f] “Non-Accepted Answers” counts each distinct user who authored answers that were \emph{not accepted} and groups them by how many non-accepted answers they authored.
\end{tablenotes}
\end{threeparttable}
\end{table}
\begin{tcolorbox}[colback=black!10!white,colframe=black]
\textbf{Findings:} 
\textcolor{blue}{Our analysis reveals a proportional trend between logging questions and user engagement on Stack Overflow, with many contributors providing accepted answers, though most participate only once. A similar engagement pattern is observed for Continuous Integration and refactoring on Stack Overflow. Distinctively, logging emerges as a cross-cutting topic, spanning programming languages, frameworks, DevOps tools, machine learning, and security. This hybrid nature sets it apart from Continuous Integration, which is infrastructure-driven, and refactoring, which is programming language and design driven, underscoring logging’s widespread and evolving relevance across diverse technological domains.}  
\end{tcolorbox}

\subsection{RQ2: Popular Topic of Logging}
\label{sec:RQ2}

\textcolor{blue}{We utilized an LLM-based approach to identify prevalent topics within Stack Overflow logging discussions. This method allowed us to classify discussions into well-defined topics based on both the title and body of the posts. As shown in \autoref{fig:horizontal_topic}, the analysis revealed 11 distinct topics. \textit{General Logging Practices} emerged as the most discussed topic, comprising \textbf{36.53\%} of questions (78{,}939 of 216{,}094). It is followed by \textit{Error Handling and Debugging} at \textbf{21.27\%} (45{,}963) and \textit{Logging Levels and Output} at \textbf{14.54\%} (31{,}420). A further \textbf{14.30\%} (30{,}901) of posts concern \textit{File Logging and Configuration}. The remaining topics each account for less than 5\% of questions: \textit{Custom Logging Frameworks} (4.26\%), \textit{Data and TensorBoard Logging} (2.56\%), \textit{Logging in Containerized Environments} (2.36\%), \textit{Logback and Application Configuration} (1.42\%), \textit{Event Logging and Monitoring} (1.12\%), \textit{NLog and .NET Logging} (0.92\%), and \textit{Testing and CI Pipelines} (0.71\%). 
These topic distributions can also be understood in light of RQ1 (Section \ref{sec:RQ1}). As seen in \autoref{fig:popularity}, logging discussions grew steadily until 2020 before plateauing and later declining, a shift mirrored in the declining adoption of dominant tags such as Java and Log4j. This temporal contraction helps explain why only a small subset of topics, such as \textit{General Logging Practices}, \textit{Error Handling and Debugging}, and \textit{Logging Levels and Output}, continued to dominate discussions, because they (i) recur across stacks and skill levels, (ii) are tightly coupled to day-to-day development (configuration, failure diagnosis, message/level choices), while specialized areas like \textit{Data and TensorBoard Logging} and \textit{Event Logging and Monitoring} remained relatively marginal, because they (a) involve narrower practitioner populations (ML practitioners) and (b) depend on tool-specific ecosystems (TensorBoard,MLflow). Moreover, the tag analysis in RQ1 \autoref{fig:tags} showed that programming concepts (40\%) and frameworks/libraries (14.9\%) dominate the ecosystem of logging-related discussions. These broad categories strongly overlap with the most prevalent topics identified.
In the following, we detail each topic and provide representative questions.}

\textcolor{blue}{\textit{\textbf{1. General Logging Practices (36.53\%).}} This is the most discussed topic (\autoref{fig:horizontal_topic}), includes questions related to the general usage of logging across various programming languages such as Python (e.g., $Q_{\text{id}}$: 78901762) \citep{stack5}, JAVA (e.g., $Q_{\text{id}}$: 4587174) \citep{stack6}, .NET (e.g., $Q_{\text{id}}$: 78860915) \citep{stack7}, and Android (e.g., $Q_{\text{id}}$: 5190860) \citep{stack8}. Previous studies have characterized logging practices in popular programming languages including Java \citep{chen2017characterizing}, Android \citep{zeng2019studying}, C/C++ \citep{yuan2012characterizing}, identifying pervasive trends and common challenges. As a significant area of interest in logging-related discussions, there is a clear need for more educational resources on the usage and implementation of logging across different facets of programming. \\ 
\textit{\textbf{2. Error Handling and Debugging (21.27\%).}} This topic, highlighted as the second most popular in \autoref{fig:horizontal_topic}, includes challenges and errors faced by practitioners when implementing logging in their projects. Questions such as (e.g., $Q_{\text{id}}$: 78819869) \textit{``Logging issue in my application after migrating from Wildfly 18 to 33"} and (e.g., $Q_{\text{id}}$: 78965763) \textit{``logging/print statements not being captured when running script with Runas command"} exemplify the difficulties encountered. Similar to previous studies \citep{li2020qualitative}, other questions in this category draw connections between logging and debugging, such as (e.g., $Q_{\text{id}}$: 78901762) \textit{``Visual Studio Console Debug Popup"} and (e.g., $Q_{\text{id}}$: 78901762) \textit{``Intellij IDEA getting remote logs while debugging"}. These inquiries highlight practitioners' awareness of the critical role that logging plays in the debugging process.\\ 
\textit{\textbf{3. Logging Levels and Output (14.54\%).}} This topic focuses on choosing log levels (DEBUG/INFO/WARN/ERROR) and composing messages/dynamic fields. Previous research indicates that setting the appropriate log level, message, and dynamic variables presents significant challenges for logging practitioners \citep{li2017log,anu2019approach,li2020towards}, which explains why practitioners often turn to Stack Overflow for assistance. Typical queries include issues related to log levels (e.g., $Q_{\text{id}}$: 2031163; 71354500) \citep{stack1,stack2}, log messages (e.g., $Q_{\text{id}}$: 14058453) \citep{stack3}, and dynamic variables (e.g., $Q_{\text{id}}$: 78958199) \citep{stack4}.\\
\textit{\textbf{4. File Logging and Configuration (14.30\%).}} This topic focuses on the technical aspects of managing and configuring log files effectively. It includes common questions related to the organization and storage of log data, such as (e.g., $Q_{\text{id}}$: 78743357) \textit{``How to Archive log4net Logs to an Archive Folder with Date and Time in Filename?"} which involves time-stamped log archiving. Other inquiries like (e.g., $Q_{\text{id}}$: 78972736) \textit{``Splitting up the Log Files in Log4j2?"} address the partitioning of logs for better manageability and performance. Additionally, questions such as (e.g., $Q_{\text{id}}$: 78979109) \textit{``Logs not being written if the parent directory is included in the filename"} reflect challenges in log file path configurations.\\
\textit{\textbf{5. Custom Logging Frameworks (4.26\%).}} This topic explores how practitioners often require or develop custom logging solutions in response to the unique needs of their applications. For example, developers seek guidance on integrating custom functionality within established logging libraries, as evidenced by questions like (e.g., $Q_{\text{id}}$: 78863938) \textit{``Is it possible to access the logger name in a custom logproc of the Tcl logger library?"} and (e.g., $Q_{\text{id}}$: 78753528) \textit{``How to use a custom DB logger with TypeORM?"}. These queries highlight the need for customization in logging practices, allowing for enhanced functionality such as accessing logger attributes or integrating logging with database management systems. Furthermore, even within widely used languages like Python, there is a demand for adapting traditional logging approaches to suit specific project requirements. An illustrative question from the SO community is (e.g., $Q_{\text{id}}$: 78613726) \textit{``Python custom logger multiple modules with variable logger name"} \citep{stack9}, where the challenge lies in extending the Python logging library to handle variable logger names across multiple modules. This topic underscores the ongoing need for flexible logging solutions that can adapt to diverse development environments and requirements.\\
\textit{\textbf{6. Data and TensorBoard Logging (2.56\%).}} Here, discussions are related to logging within data-intensive systems, particularly those involving machine learning applications. Practitioners explore tools like TensorBoard \citep{TensorBoard} and MLflow \citep{MLflow} to effectively manage and visualize logs in such environments. Questions such as (e.g., $Q_{\text{id}}$: 70478173) \textit{``How to track the big data stored in Gdrive through DVC?"}, (e.g., $Q_{\text{id}}$: 78753528) \textit{``Why does tensorboard not show all metrics?"}, (e.g., $Q_{\text{id}}$: 72684326) \textit{``How to change Sklearn flavors version in mlflow on azure machine learning?"}, underscore the complexity and the specific needs of logging in ML-based applications. The popularity of TensorBoard as a logging tool highlights its significance in providing insights that are crucial for the optimization and tuning of machine learning models. Representing 5.21\% of logging discussion on SO, there is a need for further research to investigate challenges faced by ML practitioners in logging practice. Recent studies, begin to address these gaps by investigating logging practices in ML-based applications \citep{foalem2024studying}.\\
\textit{\textbf{7. Logging in Containerized Environments (2.36\%).}} As depicted in Figure \ref{fig:tags_concepts}, logging has been associated with a variety of technologies and concepts, including concepts around containerized environments. Containerization technologies such as Docker and Kubernetes have revolutionized deployment practices, necessitating sophisticated logging mechanisms as highlighted by many previous studies \citep{alves2021identifying, chen2020docker}. Questions such as (e.g., $Q_{\text{id}}$: 78934939) \textit{``Filebeat: Not able to scrape logs of Spark on Kubernetes"} and (e.g., $Q_{\text{id}}$: 75725865) \textit{``How to Prevent Docker Container Logs from Disappearing?"} reflect common concerns about capturing and preserving logs in these environments. These discussions highlight the need for robust logging solutions that can adapt to the complexities of container orchestration, ensuring that logs are accessible and meaningful for debugging and monitoring distributed applications. \\
\textit{\textbf{8. Logback and Application Configuration (1.42\%).}} Logback, is a Java logging framework, that often requires extensive configuration to effectively manage log outputs, particularly when integrated with frameworks like Spring Boot. which frequently prompts developers to seek assistance from SO community. Common challenges include issues like (e.g., $Q_{\text{id}}$: 78441955) \textit{``Logback Spring Boot configuration is not working on Azure"}. Developers also encounter problems with basic Logback setups in Java applications, as seen in posts like (e.g., $Q_{\text{id}}$: 54467849) \textit{``Java based Logback Configuration"}\citep{stack10}. Moreover, the need for dynamic logging configurations leads to questions such as (e.g., $Q_{\text{id}}$: 77171429) ``How do I programmatically tell Logback 1.4.x to Reload Configuration?''. This ongoing dialogue within the SO community illustrates the indispensable role of peer support in overcoming the intricacies of Logback configuration.\\
\textit{\textbf{9. Event Logging and Monitoring (1.12\%).}} Event logging plays a pivotal role in monitoring applications by capturing and recording key events that occur within software systems. These logs are crucial for diagnosing issues, understanding software behavior, and improving system reliability. Prior research \citep{cinque2012event,vaarandi2008mining,
liang2007failure}, has highlighted the significance of event logs in analyzing software failures and enhancing fault diagnosis processes. In practical terms, developers are often confronted with specific challenges related to event logging, such as ensuring the synchronization of clock settings in distributed environments, as questioned in \textit{``Do AWS CloudWatch Logs Events have a Synchronized Clock?"} (e.g., $Q_{\text{id}}$: 52488775). Additionally, developers encounter issues with how event information is structured and recorded, exemplified by \textit{``OpCode is being attached to event name in out-of-process Semantic Logging (SALB) C\#"} (e.g., $Q_{\text{id}}$: 41671072). These inquiries illustrate the ongoing need to refine event logging techniques to support effective monitoring and fault resolution strategies in complex software environments.\\
\textit{\textbf{10. NLog and .NET Logging (0.92\%).}} This topic encompasses specialized discussions focused on leveraging the NLog library within .NET applications, addressing issues specific to this popular logging framework. For instance, developers encounter challenges such as configuring NLog to work effectively in modern frameworks, exemplified by the query (e.g., $Q_{\text{id}}$: 63065604) \textit{``NLog target database not working in ASP.NET Core 2.2 MVC"}.\\
\textit{\textbf{11. Testing and CI Pipelines (0.71\%).}} The integration of logging within testing and continuous integration (CI) pipelines is a critical intersection of development practices, aimed at enhancing diagnostic capabilities and ensuring robust software delivery. Although this is the least-discussed topic in our corpus, prior research has begun to tackle logging within test code and testing workflows (e.g., \citep{zhang2022studying}). This topic explores questions related to capturing and analyzing logs generated during automated testing and CI processes. For instance, developers inquire about issues such as \textit{``Where are the Selenium Logs when running in Azure DevOps Server"} (e.g., $Q_{\text{id}}$: 58218200) and how to \textit{``Customize Selenium logs for failed tests"} (e.g., $Q_{\text{id}}$: 39725477), which pertains to automated testing using the Selenium framework. Additionally, there is interest in real-time logging during test execution, as evidenced by queries like \textit{``jest, logging success or failure between each test while the tests are running"} (e.g., $Q_{\text{id}}$: 48417643). These discussions underscore the evolving role of logging in providing transparency and accountability in automated testing environments, which are crucial for troubleshooting and refining the CI/CD pipelines.\\}
\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{horizontal_percentage_plot.pdf}
    \caption{Logging topics by the percentage of their corresponding questions.}
    \label{fig:horizontal_topic}
\end{figure}

\begin{tcolorbox}[colback=black!10!white,colframe=black]
\textbf{Findings:}
\textcolor{blue}{We identified 11 topics related to logging. \textit{``General Logging Practices''} emerged as the most discussed topic, while \textit{``Testing and CI Pipelines''} was the least discussed. The top three topics (\textit{``General Logging Practices''}, \textit{``Error Handling and Debugging''}, \textit{``Logging Levels and Output''}) collectively account for 72.34\% of the entire discussion on logging; adding \textit{``File Logging and Configuration''} brings the top four to 86.64\%.}
\end{tcolorbox}

\subsection{RQ3: Logging Challenges}
\label{sec:RQ3}
\textcolor{blue}{\autoref{tab:popular_difficulty} presents the results on topic popularity and difficulty. Popularity is quantified through two metrics: Average Views (Avg. Views) and Average Scores (Avg. Scores), whereas difficulty is assessed by the percentage of questions without accepted answers (No Acc. Answers \%), the percentage of unanswered questions (No Answers \%), and the median time to receive an accepted answer (Median Hours to Acc. Answer). These metrics and approaches are based on the methodologies presented in previous studies \citep{openja2020analysis, peruma2022refactor, ouni2023empirical}.}

\textcolor{blue}{\textbf{Popularity:} As observed in \autoref{tab:popular_difficulty}, the topic ``Logging Levels and Output'' emerges as the most popular, with the highest average score of 4.13 and average views of 4825.73. In contrast, ``Data and Tensorboard Logging'' ranks as the least popular, closely followed by ``Event Logging and Monitoring''. ``Logback and Application Configuration'' and ``File Logging and Configuration'' also show high popularity, exhibiting significant viewership as depicted in Figure \ref{fig:bubble}.
These trends align with findings from prior studies on logging practices. For instance, researchers have noted that developers often struggle to determine appropriate log verbosity levels, making configuration of log levels a frequent topic of discussion \citep{li2017log, anu2019approach, kim2020automatic, li2020qualitative}. Likewise, the prominence of ``Logback and Application Configuration'' corresponds to the widespread adoption of the Logback framework in industry in 2024; over half of Java applications used Logback, which naturally leads many practitioners to seek guidance on configuring this tool \citep{NewRelic}.
``Data and TensorBoard Logging'' appears to be the least popular topic, suggesting that logging in data-driven systems is a niche concern among practitioners. Empirical studies have found that logging is less pervasive in machine learning-based applications than in traditional software \citep{foalem2024studying}. Meanwhile, the relatively lower interest in ``Event Logging and Monitoring'' may indicate that advanced log monitoring is a more specialized challenge, echoing observations that deriving insights from logs at scale remains difficult in practice \citep{candido2021log}.
In the CI study \citep{ouni2023empirical}, the most popular topics were ``Build'' and ``Culture'', both of which attracted the highest attention, with average scores of 3.28-3.23 and views 2488.8-2082.8, respectively. These results reflect CI’s strong association with infrastructure and platform-oriented practices.
In the Refactoring study \citep{peruma2022refactor}, popularity was concentrated on ``Architecture and Design Patterns'' and ``Unit Testing'', which reached the highest average views (2383.3 and 2188.7) and scores (1.25-1.26). This pattern aligns with refactoring's language and design-centric nature, emphasizing code optimization, testing, and design best practices.\\
When comparing average popularity across the three domains, logging emerges as the most popular overall, with an average of 3550.56 views per topic and an average score of 2.67. This surpasses both refactoring, which averages 2747.3 views and a score of 1.25, and CI, which averages only 1996.5 views and a score of 2.94. These indicate that logging discussions attract broader developer attention than either CI or refactoring.}

% likely due to logging’s cross-cutting nature across programming languages, frameworks, and platforms. While CI popularity is tied primarily to infrastructure tools and refactoring is centered on language-specific code transformations, logging’s hybrid scope ensures its consistent visibility and relevance across diverse technological contexts.
% As observed in \autoref{tab:popular_difficulty}, the topic ``Logging in Containerized Environments" emerges as the most popular, with the highest average score of 6.43\% and average views of 7614.97. In contrast, ``Event Logging and Monitoring'' ranks as the least popular. ``Logback and Application Configuration'' and ``Logging Levels and Output'' follow closely in popularity, exhibiting significant viewership as depicted in Figure \ref{fig:bubble}.
\textcolor{blue}{\textbf{Difficulty:} Regarding question difficulty, as shown in \autoref{tab:popular_difficulty} and illustrated in Figure~\ref{fig:bubble}, ``Logging in Containerized Environments'' is the most difficult topic: it has the highest share of questions without accepted answers (64.91\%) and the largest unanswered proportion (22.96\%), with a relatively long median time to acceptance (47.32 hours). The second most difficult topic by the same criterion is ``Testing and CI Pipelines'', with 59.92\% of questions lacking an accepted answer and a median of 48.54 hours. ``Logback and Application Configuration'' ranks third on this difficulty metric (59.65\% without accepted answers) and is distinctive for having by far the longest median time to an accepted answer (118.14 hours), pointing to persistent configuration challenges despite Logback’s wide use in the JAVA programming language \citep{NewRelic}. 
At the other end of the spectrum, ``NLog and .NET Logging" appears the least difficult, with the lowest rate of questions without accepted answers (50.35\%) and a relatively long median resolution time (74.89 hours). ``General Logging Practices'' is also among the least difficult, showing a near-lowest rate (51.56\%) and the shortest median resolution time (21.36 hours). ``Custom Logging Frameworks'' follows closely with 51.65\% of questions lacking accepted answers. By contrast, ``Data and Tensorboard Logging'' though among the least popular, shows 59.06\% without accepted answers and a median of 22.00 hours, indicating that while questions are fewer, they are typically resolved relatively quickly when they arise.
``Logging Levels and Output'' also stands out as both the most popular topic and one of the least difficult ones. It attracts the highest attention from developers in terms of average score (4.13) and views (4825.73), yet only 52.37\% of its questions remain without accepted answers, and the fewest unanswered questions (15.49). This dual status reflects the fact that, while developers frequently discuss when to use levels such as DEBUG, INFO, WARN, or ERROR, the community is often able to provide guidance. The relative ease of resolving such questions is consistent with prior academic work: early research adopted machine learning to predict appropriate logging levels automatically, framing log severity assignment as a classification problem and demonstrating that patterns of log-level usage can be effectively learned from code repositories \citep{li2017log,zhu2015learning}.
When compared with related domains. In the CI study \citep{ouni2023empirical}, the most difficult topics were ``Version Control'' (59\% without accepted answers) and ``Deployment'' (58\%), while ``Testing'' had the longest median time to an accepted answer (18 hours).
In the refactoring study \citep{peruma2022refactor}, the most difficult topic were ``Tools and IDEs'' (42.34\% without accepted answers) and ``Unit Testing'' (37.78\%), while ``Database'' showed the longest median time to receive an accepted answer (0.44 hours). \\
Taken together, these comparisons reveal that logging-related discussions emerge as the most difficult and time-consuming, with an average of 56.49\% of questions lacking accepted answers and a median of 45.37 hours to reach resolution. CI questions are similarly difficult in terms of unresolved proportion (54\%), but they are typically resolved much faster, with a median time of only 11 hours. In contrast, ``Refactoring'' appears considerably less difficult overall, with just 36.58\% of questions lacking accepted answers and an extremely short median resolution time of 0.39 hours.}

% Overall, CI discussions appear more tractable, with an average of 54% of questions lacking accepted answers and a median response time of 11 hours, suggesting that despite integration complexity, solutions are often quickly identified.
% questions about ``Logging in Containerized Environments" are the most challenging based on our logging dataset extracted from SO. They have the highest percentage of questions without accepted answers at 64.52\%, the second-highest percentage of unanswered questions at 23.12\%, and also feature the third-longest median response time among all categories examined. It is important to note that while ``where to log?" is a critical area of study in academic research, it is seldom questioned by developers in community-driven Q\&A platforms like Stack Overflow, possibly due to the prevalence of established logging practices and comprehensive documentation available within current logging frameworks." ``Logback and Application Configuration" is the next most difficult, with 60.67\% of questions remaining without accepted answers. Conversely, ``General Logging Practices" is less challenging, with the lowest percentage of questions without accepted answers at 49.57\%. ``Testing and CI Pipelines" stands out in terms of response time, taking significantly longer twice as long on average—to receive an accepted response compared to other topics. The topic ``Data and Tensorboard Logging" shows the shortest median response time at 23 hours, likely influenced by its relevance to the rapidly evolving field of machine learning.

% \input{Table/Popularity_Difficulty}
\begin{table*}[htbp]
\centering
\caption{Popularity and difficulty of Logging topics.}
\label{tab:popular_difficulty}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Topic}} & \multicolumn{2}{c}{\textbf{Popularity Metrics}} & \multicolumn{3}{c}{\textbf{Difficulty Metrics}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-6}
 & \textbf{Avg. Views} & \textbf{Avg. Scores} & \textbf{No Answers \%} & \textbf{No Acc. Answers \%} & \textbf{Median Hours to Acc. Answer} \\
\midrule
Custom Logging Frameworks & 3195.12 & 2.90 & 16.42 & 51.65 & 29.51 \\
Data and Tensorboard Logging & 2693.67 & 2.15 & 19.48 & 59.06 & 22.00 \\
Error Handling and Debugging & 3425.10 & 2.05 & 20.43 & 58.67 & 23.83 \\
Event Logging and Monitoring & 2948.57 & 1.85 & 18.15 & 56.33 & 31.16 \\
File Logging and Configuration & 3898.75 & 2.37 & 16.38 & 57.00 & 25.54 \\
General Logging Practices & 3196.82 & 2.79 & 14.50 & 51.56 & 21.36 \\
Logback and Application Configuration & 4249.74 & 2.56 & 19.76 & 59.65 & \textbf{118.14} \\
Logging Levels and Output & \textbf{4825.73} & \textbf{4.13} & 15.49 & 52.34 & 56.83 \\
Logging in Containerized Environments & 3985.13 & 2.68 & \textbf{22.96} & \textbf{64.91} & 47.32 \\
NLog and .NET Logging & 3365.45 & 2.95 & 14.57 & 50.35 & 74.89 \\
Testing and CI Pipelines & 3272.13 & 2.91 & 17.35 & 59.92 & 48.54 \\
\midrule
\textbf{Average for all Logging topics} & 3550.56 & 2.67 & 17.77 & 56.49 & 45.37 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{bubble_plot2 (1)_cropped.pdf}
    \caption{Comparison of logging topics by popularity \& difficulty}
    \label{fig:bubble}
\end{figure}

\begin{tcolorbox}[colback=black!10!white,colframe=black]
\textbf{Findings:}
\textcolor{blue}{The topic \textit{``Logging in Containerized Environments''} stands out as the most difficult, with 64.91\% of questions lacking accepted answers and long resolution times. By contrast, \textit{“Logging Levels and Output”} emerges as both the most popular and among the least difficult. When compared across domains, logging-related discussions are relatively more difficult and time-consuming, averaging 45.37 hours to resolution, while CI achieves faster turnaround (11 hours) despite similar difficulty rates, and refactoring remains the least difficult, with only 36.58\% unresolved and an average of 0.39 hours to resolution.}
\end{tcolorbox}


==> 6_Related_work.tex <==
In this section, we introduce and discuss two areas of related works: (i) research done on logging characteristics, and (ii) research done on developers' challenges.  
\subsection*{\textbf{Studies on characterizing logging practice:}}
\textcolor{blue}{Logging practices are essential across the software development lifecycle, impacting both traditional software engineering and ML/AI applications. Studies \citep{batoun2024literature, he2022empirical, yang2023interview, gu2022logging} show logging's extensive role in capturing execution details and behavior in various environments. Effective logging has been proven to reduce debugging time and improve diagnostics \citep{kabinna2018examining, li2020qualitative, gu2022logging}. Logging also plays a vital role in software testing, facilitating the identification and analysis of test failures \citep{zhang2022studying}.}

\textcolor{blue}{In ML/AI, logging adapts to challenges like complex models and large datasets. Foalem et al. \citep{foalem2024studying} highlight the development of ML-specific tools such as MLflow and TensorBoard, which enhance functionality to track model performance, manage hyperparameters, and monitor training metrics, meeting the unique needs of ML applications.}

\textcolor{blue}{While these studies characterize logging practices in specific domains (general-purpose software or ML/AI), they primarily rely on project-level or tool-level data. None of them systematically investigate how logging challenges emerge and evolve across a large-scale, community-driven knowledge base such as Stack Overflow. Our study addresses this gap by examining more than 200K logging-related discussions spanning multiple ecosystems and technologies. This enables us to capture not only what logging practices exist but also how developers experience and articulate logging difficulties in practice, providing a broader, cross-domain perspective that previous studies lack.}  
\subsection*{\textbf{Studies on developers'challenges:}}
\textcolor{blue}{Understanding developer challenges is crucial for advancing software engineering and enhancing tool support. Stack Overflow, a key resource, provides insights into these challenges through user interactions. Research using Stack Overflow data \citep{barua2014developers, abdalkareem2017developers, openja2020analysis, wang2013empirical, rosen2016mobile} has revealed prevalent issues in software engineering, detailing the questions developers ask and the solutions provided. As machine learning and AI evolve, new challenges emerge. Studies \citep{islam2019developers, ahmad2020systematic, alshangiti2019developing,zhang2019empirical} have identified specific obstacles in developing and updating ML models. Additionally, Johri et al. \citep{johri2018identifying} used topic analysis to track technology and programming trends on Stack Overflow, demonstrating the impact of community-driven knowledge. A similar study has been conducted by Openja et al \citep{openja2020analysis} to understand the popularity and challenge of modern release engineering topics.
This research provides invaluable insights into the developer experience, guiding the development of tools and practices to improve productivity and problem-solving in software engineering.
Research has also investigated developer challenges in other critical areas of software engineering. Peruma et al.~\citep{peruma2022refactor} analyzed Stack Overflow posts to characterize challenges related to refactoring, showing that developers frequently struggle with tool support, migration issues, and understanding code dependencies. Similarly, Ouni et al.~\citep{ouni2023empirical} studied questions related to Continuous Integration (CI), identifying pain points in build failures, pipeline configuration, and the integration of new tools into CI environments. These works underscore that Stack Overflow serves as a valuable lens for identifying domain-specific challenges across software engineering.}  

\textcolor{blue}{Although these studies provide invaluable insights into developer challenges, they are typically domain-specific (e.g., ML/AI, mobile, release engineering) or focus on broad software engineering trends. None of them directly address logging as a first-class concern. Our work is the first to systematically investigate logging-related developer challenges on Stack Overflow. By doing so, we uncover trends, pain points, and knowledge gaps unique to logging, complementing prior studies while addressing a neglected but critical aspect of software engineering practice.}  





==> 7_Discussion_Implication.tex <==
We describe the implications of our findings for practitioners, researchers, framework vendors, and educators aiming to improve logging frameworks and practices.

\textbf{Implication for  Researchers.} The results of our study highlight the significant attention that logging practices are receiving across various technology domains, revealing a wide spectrum of challenges that developers encounter, as detailed in our RQ3 findings. These insights present urgent areas for research:
\begin{itemize}
    \item \textcolor{blue}{Containerized Environments: Our findings underscore that logging within containerized environments is the most challenging topic in logging discussions on Stack Overflow, as evidenced in Figure \ref{fig:bubble}. We found that this area has received some, but still limited, attention from the research community. Early effort to bridge this gap includes the work of Moilanen et al. \citep{moilanen2020collecting}, who developed a solution for collecting logs from Docker containers, and Chen et al. \citep{chen2020docker}, who explored Docker container log collection using the ELK stack (Elasticsearch, Logstash, and Kibana). Alves et al. \citep{alves2021identifying} also contributed by investigating logging practices in open-source Python containerized applications. However, despite the advancements, several key shortcomings persist. One of the primary challenges remains the ephemeral nature of containers, which often leads to log data being lost when containers are terminated, despite efforts to implement persistent logging solutions \citep{mezmo}. Additionally, while many solutions exist, such as the ELK stack, they often introduce significant overhead, which becomes problematic at scale \citep{chen2020docker}. The integration of these solutions with modern container orchestrators like Kubernetes \citep{eks}, Google Cloud \citep{Googlecloud}, Docker \citep{docker}, and AWS \citep{AWS} remains unexplored. Moreover, while existing research has made important strides, it primarily focuses on specific frameworks or tools (e.g., Docker, Kubernetes, or Python), leaving gaps in understanding for newer or hybrid technologies, such as multi-cloud setups, serverless containers (e.g., AWS Fargate), and microservices architectures transitioning from monolithic systems. Finally, security and isolation of logs, particularly in multi-tenant environments, remain a critical challenge that has not been fully addressed in current solutions \citep{mezmo}. These gaps present opportunities for future research and improvements in containerized logging practices.}
    \textcolor{blue}{\item Broadening the scope to other fields: Logging is integral to many well-established fields such as machine learning, databases, DevOps, and security, as shown in Figure \ref{fig:tags_concepts}. However, these critical areas receive limited attention from academia, impacting the effectiveness with which practitioners manage logging challenges. Evidence from Table \ref{tab:popular_difficulty} show that  “Testing and CI Pipelines”  exhibits a high unresolved rate (59.92\%) and the second-longest median time to an accepted answer (48.54 h), while typical CI questions resolve far faster (≈ 11 h in \cite{ouni2023empirical}). This disparity indicates that when CI problems involve logging, they are materially harder. We therefore encourage future work on \texttt{logging for Testing \& CI Pipelines} to be situated within the CI topical taxonomy identified by prior CI research--e.g., Build, Version Control, Deployment, Testing, and Culture \cite{ouni2023empirical}--and to examine the role of logging within each topic. Complementarily, researchers should investigate how effective logging mitigates risks in database management and prevents data leaks in ML-intensive systems. These studies could provide new insights that directly impact and improve logging practices across these various domains.}


% Broadening the scope to other fields: Logging is integral to many well-established fields such as machine learning, databases, DevOps, and security, as shown in Figure \ref{fig:tags_concepts}. However, these critical areas receive less attention from academia, impacting the effectiveness with which practitioners manage logging challenges. For example, as detailed in Table \ref{tab:popular_difficulty}, the “Testing and CI Pipelines” topic has the longest median time to receive an accepted answer on Stack Overflow, indicating substantial difficulties that could significantly benefit from focused research efforts. Concrete studies or specific research questions could explore how logging practices can be optimized in CI/CD pipelines or how effective logging can mitigate risks in database management and data leaks in intensive machine learning systems. These studies could provide new insights that directly impact and improve logging practices across these various domains.
\end{itemize}

\textbf{Implication for Practitioners.} Our study clearly indicates which logging topics are most challenging within the development community, guiding team leaders in effectively allocating resources and tasks among their project teams. Based on our findings, certain areas such as \textit{Logging in Containerized Environments}, \textit{Logback and Application Configuration}, \textit{Testing and CI Pipelines}, \textit{Data and Tensorboard Logging}, and \textit{Error Handling and Debugging} have proven to be particularly complex as show in \autoref{fig:bubble}. These topics consistently exhibit higher difficulties, as reflected by the high percentage of questions without accepted answers and longer median response times. Given that logging tasks are often intertwined with broader coding responsibilities, it is advisable for team leaders to involve the most skilled and experienced developers in reviewing and overseeing logging-related activities within these complex areas. Experienced developers possess a deeper understanding of system architecture, potential pitfalls, and advanced debugging techniques vital to efficiently managing complex logging tasks. This approach not only ensures that logging is effectively integrated into the development process but also leverages the expertise of experienced developers to mentor others, enhancing overall code quality and maintainability. 
\textcolor{blue}{Our analysis (see \autoref{fig:popularity}, \autoref{tab:popular_tags}, \autoref{fig:tags}) shows that most logging activity is concentrated in the Java Virtual Machine (JVM) ecosystem (\texttt{Java}, \texttt{log4j}/\texttt{log4j2}, \texttt{logback}). Significant activity also appears in \texttt{Python}, \texttt{C\#}, and \texttt{JavaScript}, while observability tools such as \texttt{logstash} peaked in popularity during the mid-2010s. Logging practices also spread across many other technologies (\autoref{fig:tags_concepts}). For small teams with limited senior expertise, we recommend focusing on the ecosystem that dominates the codebase, typically one of the dominant ecosystems highlighted in our analysis (e.g., JVM-based frameworks, Python, C\#, or JavaScript). To simplify adoption, teams should begin with well-tested configuration templates for that stack, enforce a minimal baseline for logging to reduce setup complexity, and rotate a lightweight ``logging champion" role to review pull requests involving logging. These practices enable less-experienced developers to maintain reliable logging without requiring deep prior expertise.}
 
\textbf{Implication for Logging Framework Vendors.} Our analysis reveals that certain logging frameworks, notably TensorBoard, and Logback, consistently appear in the context of challenging discussions, as evidenced by \autoref{fig:bubble}. These frameworks are associated with topics that have been identified as particularly problematic, reflecting a broader need within the community for better support and documentation.
\begin{itemize}
    \item Enhanced Documentation: The prevalent discussion around \textit{Logging Levels and Output} and \textit{General Logging Practices}, as depicted in Figure \ref{fig:horizontal_topic}, underscores the necessity for framework vendors to substantially improve their documentation. This should comprehensively cover foundational logging concepts such as operational guidelines (how, what, and where to log) and strategic advice on setting log levels, areas that dominate SO discussions \citep{stackoverflow001}.
    \textcolor{blue}{\item Customization Needs: With 4.26\% of all logging discussions focusing on custom logging frameworks, there is a clear demand for frameworks that offer higher levels of customization. Framework vendors should consider developing more flexible logging solutions that can be easily tailored to meet the diverse and specific requirements of developers. Key customization needs include: \texttt{Message formatting} -- adding contextual information (e.g., session IDs or environment variables) to each log entry, as seen in discussions on extending Log4j2 \citep{stackoverflow50241376}. \texttt{Configuration flexibility} -- enabling support for non-standard configuration formats (e.g., JSON instead of XML in Log4j2) \citep{stackoverflow32269559}. \texttt{Framework interoperability} -- adapting one framework’s logger (e.g., Pino) to work with other tools such as TypeORM or external observability pipelines \citep{stackoverflow65407405}.} 
    \item Domain-Specific Frameworks: The intersection of logging with various specialized domains, including machine learning, databases, CI/CD, and security, presents a unique opportunity for the creation of domain-specific logging frameworks. Such specialized tools would cater to the unique challenges and needs of these fields, potentially transforming logging practices in these areas.
\end{itemize}


\textbf{Implications for Educators:} Our study has identified several logging topics that are prominently discussed on Stack Overflow, which should inform the curricula of training programs and educational materials. Topics such as  \textit{``Logging Levels and Output", ``General Logging Practices", ``Error Handling and Debugging",} and \textit{``File Logging and Configuration,"} represent a significant portion of the logging-related queries. These areas have also been the subject of extensive research, reflecting their importance and complexity in software development. As such, they should be covered extensively in educational programs to equip learners with the necessary skills to address common logging issues effectively. This integration of practical query data with academic insights can help ensure that educational materials are both comprehensive and directly relevant to the needs of the industry.

Moreover, special attention should be given to \textit{``Data and Tensorboard Logging"} and \textit{``Testing and CI Pipelines"} which are connected to the dynamic fields of machine learning and software testing. These topics are becoming increasingly important within the logging sphere, reflecting the evolving nature of technology and the need for specialized knowledge in these areas. Despite their growing importance, there has been comparatively less research tackling these specific challenges directly. This gap highlights an opportunity for academic environments to pioneer research and educational content that addresses these cutting-edge topics. Educators are encouraged to integrate these subjects into their teaching materials to prepare students for the challenges they will face in modern software environments \citep{microsoft1}.

==> 8_Threats_to__validity.tex <==
In this section, we discuss the potential threats to the validity of our research
methodology and findings.

\textbf{Selection of Tags:} Our method of identifying relevant discussions through pre-selected tags and keyword-matching mechanisms might introduce biases. This approach may overlook certain posts that discuss relevant issues but do not use the specific tags or keywords we selected. Although we aim to capture a comprehensive range of challenges by focusing on popular and widely used terms, there is a risk of missing discussions that either use less common terminology or discuss emerging issues not yet well-represented by our chosen keywords.

\textbf{Reliance on a Single Data Source:} By relying solely on Stack Overflow as the data source, we may miss insights available in other forums, blogs, or publications where developers discuss challenges in logging within ML environments. Although Stack Overflow is a rich and diverse platform used by both novice and expert developers, extending our data sources could provide a more rounded view of the challenges faced in this domain.

\textbf{Impact of External Factors on Logging Practices:} Our study, while extensive, does not account for the specific technological, tool-based, or business system contexts within which logging practices are implemented. The variability in logging statements and practices can be profoundly influenced by the underlying technology stack, the tools employed, and the business requirements driving the system designs. As such, the generalizability of our findings may be limited by our dataset's lack of detailed context about the specific environments in which the logging occurs. Future research could enhance the validity of findings by incorporating studies that link logging practices directly to specific types of technology stacks and business applications, providing a richer, more nuanced understanding of the challenges and practices in diverse development environments.

\textbf{Subjectivity in Data Analysis:} \textcolor{blue}{A potential threat arises from the inherent subjectivity involved in defining and categorizing topics from Stack Overflow discussions. To mitigate this, we adopted a structured ground-truth construction process aligning with the methodology of the previous study \citep{abbassi2025unveiling, verdet2023exploring}: two PhD researchers with over six years of experience in software engineering collaboratively applied open coding to a 10\% pilot sample of posts. This process iteratively refined the taxonomy of topics until convergence on 11 stable categories. To further ensure robustness, the two authors independently labeled the final 50\% of the dataset, reaching a substantial inter-rater reliability with a Cohen’s Kappa score of 0.781. Disagreements were resolved through consensus discussions. This reliability check reduces the risk of individual bias and is consistent with best practices in empirical software engineering research \citep{foalem2024studying, abbassi2025unveiling, foalem2025logging}. Another threat comes from the use of an LLM (GPT-4o-mini) as a “judge” for topic classification. While LLMs can capture semantic nuances beyond traditional approaches, they may also introduce risks of hallucination, prompt sensitivity, or bias inherited from their training data. We mitigated these risks in several ways: (i) we employed a reference-based judging approach \citep{lin2024engineering}, anchoring the LLM’s outputs to the manually validated taxonomy of 11 topics; (ii) we set the temperature to 0 to enforce determinism and reproducibility of outputs, following prior recommendations \citep{verdet2023exploring}; and (iii) we explicitly embedded brief descriptions of each topic in the prompt to reduce the likelihood of hallucinated or irrelevant categories \citep{sollenberger2024llm4vv}.}

% The process of categorizing and interpreting Stack Overflow posts inherently involves subjectivity. To mitigate this, we employed a hybrid approach combining an LLM-based classification method with a manually validated ground-truth sample aligning with the methodology of the previous study \citep{abbassi2025unveiling, verdet2023exploring}.


% The process of categorizing and interpreting topics from Stack Overflow posts inherently involves subjectivity. To mitigate this and ensure robustness in our classification, two reviewers analyzed the data independently. We achieved substantial inter-rater reliability with a kappa score of 0.71, indicating a high level of agreement among reviewers. Disagreements were resolved through discussions involving a third researcher, ensuring a consensus-based approach to classifications. This method of resolving differences through discussion until consensus is reached is supported by similar methodologies adopted in previous studies \citep{openja2020analysis, ouni2023empirical}. 
% Additionally, another potential threat to validity in our study comes from the use of the Latent Dirichlet Allocation (LDA) model to identify topics. The selection of the number of topics (K) and the number of iterations (I) can significantly influence the results. To address this, we adopted a robust methodology for choosing these parameters, drawing from established best practices in the literature \citep{openja2020analysis, ouni2023empirical, peruma2022refactor} and conducting multiple experiments to determine reasonable values for K and I. Furthermore, to mitigate the inherent randomness associated with LDA, we ran our final model several times to check for consistency in the topics extracted. Our analyses consistently showed minimal variation across different runs, supporting the stability and reliability of our topic modeling approach.

\textbf{Threats to Measurement Interpretation}: In RQ3, we assess the challenge of logging topics based on metrics such as view count, score, and the presence or absence of accepted answers on Stack Overflow. While these metrics are indicative and widely used in empirical software engineering research, they might not comprehensively capture the actual challenge of a topic or the complexity of the questions posed. For example, a high view count could indicate general interest but does not necessarily correlate directly with the inherent complexity of the topic. Similarly, the absence of an accepted answer could be due to several factors unrelated to the difficulty of the question, such as the specificity of the problem, the lack of engagement from the community, or even the question's clarity.




==> Table/Popular_tags.tex <==
\begin{table}[htbp]
\centering
\caption{Top-10 most popular tags.}
\label{tab:popular_tags}
%\begin{adjustbox}{width=0.6\textwidth}
\begin{tabular}{@{}lrr@{}}
\toprule
Tag          & Occurrence & Percentage \\ \midrule
% logging      & 48,965     & 7.24\%    \\
java         & 32,640     & 4.82\%     \\
log4j        & 18,647      & 2.75\%     \\
python       & 17,037      & 2.52\%     \\
c\#          & 14,795      & 2.18\%     \\
javascript       & 11,633      & 1.72\%     \\
php      & 9,007      & 1.33\%     \\
android        & 9,002      & 1.33\%     \\
log4j2         & 8,815      & 1.30\%     \\
logstash  & 8,775      & 1.29\%     \\ 
logback  & 7,259      & 1.07\%     \\ \bottomrule
\end{tabular}
%\end{adjustbox}
\end{table}

==> Table/Popularity_Difficulty.tex <==
\begin{table*}[htbp]
\centering
\caption{Popularity and difficulty of Logging topics.}
\label{tab:popular_difficulty}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Topic}} & \multicolumn{2}{c}{\textbf{Popularity Metrics}} & \multicolumn{3}{c}{\textbf{Difficulty Metrics}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-6}
 & \textbf{Avg. Views} & \textbf{Avg. Scores} & \textbf{No Answers \%} & \textbf{No Acc. Answers \%} & \textbf{Median Hours to Acc. Answer} \\
\midrule
Custom Logging Frameworks & 3195.12 & 2.90 & 16.42 & 51.65 & 29.51 \\
Data and Tensorboard Logging & 2693.67 & 2.15 & 19.48 & 59.06 & 22.00 \\
Error Handling and Debugging & 3425.10 & 2.05 & 20.43 & 58.67 & 23.83 \\
Event Logging and Monitoring & 2948.57 & 1.85 & 18.15 & 56.33 & 31.16 \\
File Logging and Configuration & 3898.75 & 2.37 & 16.38 & 57.00 & 25.54 \\
General Logging Practices & 3196.82 & 2.79 & 14.50 & 51.56 & 21.36 \\
Logback and Application Configuration & 4249.74 & 2.56 & 19.76 & 59.65 & \textbf{118.14} \\
Logging Levels and Output & \textbf{4825.73} & \textbf{4.13} & 15.49 & 52.34 & 56.83 \\
Logging in Containerized Environments & 3985.13 & 2.68 & \textbf{22.96} & \textbf{64.91} & 47.32 \\
NLog and .NET Logging & 3365.45 & 2.95 & 14.57 & 50.35 & 74.89 \\
Testing and CI Pipelines & 3272.13 & 2.91 & 17.35 & 59.92 & 48.54 \\
\midrule
\textbf{Average for all Logging topics} & 3550.56 & 2.67 & 17.77 & 56.49 & 45.37 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}


==> Table/Post_Distribution.tex <==
\begin{table}[htbp]
\centering
\caption{Distribution of the number of posts created by a user.}
\label{tab:post_distribution}
%\begin{adjustbox}{width=0.8\textwidth}
\begin{tabular}{@{}lrr@{}}
\toprule
\textbf{Number of posts created by a user} & \textbf{Count} & \textbf{Percentage} \\ \midrule
\multicolumn{3}{l}{\textit{Questions - total distinct users: 146,840 }} \\
1 & 111,584 & 75.99\% \\
2 & 23,871  & 16.26\% \\
3 & 5,108 & 3.48\% \\
4 & 2,775 & 1.89\% \\
5 & 1,186 & 0.81\% \\
Others & 2,316 & 1.58\% \\ \midrule
\multicolumn{3}{l}{\textit{Accepted Answers - total distinct users: 68,652}} \\
1 & 52,731 & 76.81\% \\
2 & 11,284 & 16.44\% \\
3 & 2,150 & 3.13\% \\
4 & 1,217 & 1.77\% \\
5 & 464 & 0.68\% \\
Others & 806 & 1.17\% \\ \midrule
\multicolumn{3}{l}{\textit{Non-Accepted Answers - total distinct users: 89,835}} \\
1 & 72,299 & 80.48\% \\
2 & 13,358 & 14.87\% \\
3 & 2,074 & 2.31\% \\
4 & 1,103 & 1.23\% \\
5 & 419 & 0.47\% \\
Others & 582 & 0.65\% \\
\bottomrule
\end{tabular}
%\end{adjustbox}
\end{table}

==> Table/Summary_Statistic.tex <==
\begin{table}[htbp]
\centering
\caption{Overview of our collected dataset.}
\label{tab:collected_data}
%\begin{adjustbox}{width=0.8\textwidth}
\begin{tabular}{@{}lr@{}}
\toprule
Metric                             & Value \\ \midrule
Number of posts                  & 216,094 \\
Number of answered posts     & 118,196 \\
Number of accepted answers       & 87,197 \\
Number of distinct tags          & 20,758 \\
Number of distinct users         & 146,840 \\
Average number of tags per question & 3 \\
Average number of answers per question & 1.35 \\ \bottomrule
\end{tabular}
%\end{adjustbox}
\end{table}

==> Table/Table1.tex <==
\begin{table}[ht]
\centering
\caption{Top-10 most popular tags of logging questions in ML-Based applications vs traditional systems}
  \label{table:top10tags}
 \begin{adjustbox}{width=0.8\textwidth}
\begin{tabular}{lcc|lcc}
\toprule
\multicolumn{3}{c|}{ML-Based Applications} & \multicolumn{3}{c}{Traditional Systems} \\
\midrule
\textbf{Tag} & \textbf{Occurrence} & \textbf{Percentage} & \textbf{Tag} & \textbf{Occurrence} & \textbf{Percentage} \\
\midrule
tensorboard & 1855 & 18.78\% & logging & 41522 & 26.07\% \\
tensorflow & 1489 & 15.07\% & java & 8235 & 5.17\% \\
python & 1164 & 11.78\% & python & 6875 & 4.32\% \\
mlflow & 734 & 7.43\% & log4j & 3356 & 2.11\% \\
keras & 292 & 2.96\% & c\# & 3217 & 2.02\% \\
machine-learning & 251 & 2.54\% & php & 1459 & 0.92\% \\
pytorch & 220 & 2.23\% & log4j2 & 1453 & 0.91\% \\
deep-learning & 176 & 1.78\% & slf4j & 1243 & 0.78\% \\
python-3.x & 153 & 1.55\% & logback & 1206 & 0.76\% \\
wandb & 144 & 1.46\% & android & 1159 & 0.73\% \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> Table/Topic_name.tex <==
\begin{table}[ht]
\centering
\caption{LDA topic Distribution and corresponding words}
\begin{adjustbox}{width=\textwidth} % Adjusted for better fit
\begin{tabular}{clm{7cm}} % Changed to 'm{8cm}' for middle vertical alignment
\hline
\textbf{Topic ID} & \textbf{Topic Name} & \textbf{Related KeyWords (unigrams \& bigrams)} \\
\hline
0 & Testing and CI Pipelines & test, training, array, pipeline, magento, engine, finding, nuget\_package, tests, javascript \\
\hline
1 & Error Handling and Debugging & error, run, get, using, code, following, im, work, version, project \\
\hline
2 & Event Logging and Monitoring & event, jar, tag, gt, correlation\_id, channel, null, integration, sentry, bundle \\
\hline
3 & File Logging and Configuration & file, log, using, configuration, want, branch, git, write, files, create \\
\hline
4 & NLog and .NET Logging & nlog, target, nlogconfig, merge, php, net\_core, elasticsearch, index, master, laravel \\
\hline
5 & Logging Levels and Output & log, message, logging, using, output, serilog, console, level, error, see \\
\hline
6 & Logging in Containerized Environments & service, sink, container, label, docker, cluster, job, endpoint, node, docker\_container \\
\hline
7 & Custom Logging Frameworks & class, using, winston, use, logger, property, method, custom, code, function \\
\hline
8 & Data and Tensorboard Logging & query, data, using, tensorboard, user, database, graph, vertex, gremlin, model \\
\hline
9 & Logback and Application Configuration & logback, application, server, dependency, project, spring\_boot, logbackxml, configuration, java, remote \\
\hline
10 & General Logging Practices & one, would, way, use, need, like, time, request, im, log \\
\hline
\end{tabular}
\end{adjustbox}
\label{tab:topic_distribution}
\end{table}

==> declaration.tex <==
\textbf{Conflicts of interest:} The authors declare that they have no conflicts of interest relevant to the content of this article.


\noindent\textbf{Funding:} Not applicable.


\noindent\textbf{Ethics approval:} Not applicable.


\noindent\textbf{Clinical Trial Number in the manuscript:} Not applicable.


\noindent\textbf{Informed Consent:} Not applicable.


\noindent\textbf{Data availability statement:} The datasets generated during and/or analysed during the current study are available in the [foalem] repository, [\url{https://shorturl.at/pOyc3}].


\textbf{Author Contributions:} 
\begin{itemize}
  \item \textbf{Patrick Loic Foalem:} Conceptualization, Data Curation, Formal Analysis, Investigation, Methodology, Visualization, Writing -- Original Draft, and Writing -- Review \& Editing.
  \item \textbf{Andre Nguimbous:} Formal analysis.
  \item \textbf{Foutse Khomh:} Project Administration, Resources, Supervision, Validation, and Writing -- Review \& Editing.
  \item \textbf{Heng Li:} Supervision and Writing -- Review \& Editing.
  \item \textbf{Ettore Merlo:} Supervision and Writing -- Review \& Editing.
\end{itemize}
% Declarations

% Funding 
% No funding was received for conducting this study.

% Conflicts of interest/Competing interests
% The authors have no relevant financial or non-financial interests to disclose.

% Availability of data and material
% The datasets generated during and/or analysed during the current study are available in the Github repository, https://github.com/senseconcordia/TestLoggingPractice.

% Code availability
% Code for data cleaning and analysis is provided as part of the replication package. It is available at https://github.com/senseconcordia/TestLoggingPractice.

% \begin{titlepage}
%     Declarations

% % Funding 
% % No funding was received for conducting this study.

% Conflicts of interest/Competing interests
% The authors declare that they have no known competing financial interests or personal relationships that could have appeared to influence the work reported in this paper.


% Code availability
% The datasets generated during and/or analysed during the current study are available in the [foalem] repository, [\url{https://shorturl.at/FLg9z}].
% \end{titlepage}
